Baryogenesis and leptogenesis with relativistic bubble walls

In this talk, we study the impact of first order phase transitions with fast bubble walls on mechanisms of leptogenesis and baryogenesis. We begin our exploration with the usual leptogenesis where the breaking of $B-L$ occurs via a PT with fast walls. Then we move to a more exotic case where the $B-L$ breaking phase transition creates heavy particles in the plasma and catalizes the leptogenesis. Finally, we apply the same production mechanism to the EWPT at low energy and build a new model of EWBG. Those models are all original and contain crucial new phenomenological aspects like the emission of large amount of Gravitational waves.

==> biblio.tex <==
@article{Dolgov:1991fr,
    author = "Dolgov, A. D.",
    title = "{NonGUT baryogenesis}",
    reportNumber = "YITP-K-940",
    doi = "10.1016/0370-1573(92)90107-B",
    journal = "Phys. Rept.",
    volume = "222",
    pages = "309--386",
    year = "1992"
}
@article{Huang:2015izx,
    author = "Huang, Fa Peng and Gu, Pei-Hong and Yin, Peng-Fei and Yu, Zhao-Huan and Zhang, Xinmin",
    title = "{Testing the electroweak phase transition and electroweak baryogenesis at the LHC and a circular electron-positron collider}",
    eprint = "1511.03969",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.93.103515",
    journal = "Phys. Rev. D",
    volume = "93",
    number = "10",
    pages = "103515",
    year = "2016"
}

@article{Delaunay:2007wb,
    author = "Delaunay, Cedric and Grojean, Christophe and Wells, James D.",
    title = "{Dynamics of Non-renormalizable Electroweak Symmetry Breaking}",
    eprint = "0711.2511",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-PH-TH-2007-219, MCTP-07-31, SACLAY-T07-141",
    doi = "10.1088/1126-6708/2008/04/029",
    journal = "JHEP",
    volume = "04",
    pages = "029",
    year = "2008"
}

@article{Chala:2018ari,
    author = "Chala, Mikael and Krause, Claudius and Nardini, Germano",
    title = "{Signals of the electroweak phase transition at colliders and gravitational wave observatories}",
    eprint = "1802.02168",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-18-241-T",
    doi = "10.1007/JHEP07(2018)062",
    journal = "JHEP",
    volume = "07",
    pages = "062",
    year = "2018"
}

@article{Gorghetto:2021fsn,
    author = "Gorghetto, Marco and Hardy, Edward and Nicolaescu, Horia",
    title = "{Observing invisible axions with gravitational waves}",
    eprint = "2101.11007",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2021/06/034",
    journal = "JCAP",
    volume = "06",
    pages = "034",
    year = "2021"
}

@article{PhysRevD.45.2685,
  title = {Electroweak phase transition and baryogenesis},
  author = {Anderson, Greg W. and Hall, Lawrence J.},
  journal = {Phys. Rev. D},
  volume = {45},
  issue = {8},
  pages = {2685--2698},
  numpages = {0},
  year = {1992},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.45.2685},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.45.2685}
}



@article{Choi:1993cv,
    author = "Choi, Jarny and Volkas, R. R.",
    title = "{Real Higgs singlet and the electroweak phase transition in the Standard Model}",
    eprint = "hep-ph/9308234",
    archivePrefix = "arXiv",
    reportNumber = "UM-P-93-80, OZ-93-20",
    doi = "10.1016/0370-2693(93)91013-D",
    journal = "Phys. Lett. B",
    volume = "317",
    pages = "385--391",
    year = "1993"
}


@article{Espinosa:1993bs,
    author = "Espinosa, J. R. and Quiros, M.",
    title = "{The Electroweak phase transition with a singlet}",
    eprint = "hep-ph/9301285",
    archivePrefix = "arXiv",
    reportNumber = "IEM-FT-67-93",
    doi = "10.1016/0370-2693(93)91111-Y",
    journal = "Phys. Lett. B",
    volume = "305",
    pages = "98--105",
    year = "1993"
}



@article{Profumo:2007wc,
    author = "Profumo, Stefano and Ramsey-Musolf, Michael J. and Shaughnessy, Gabe",
    title = "{Singlet Higgs phenomenology and the electroweak phase transition}",
    eprint = "0705.2425",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CALTECH-MAP-333, MADPH-07-1489",
    doi = "10.1088/1126-6708/2007/08/010",
    journal = "JHEP",
    volume = "08",
    pages = "010",
    year = "2007"
}



@article{Espinosa:2011ax,
    author = "Espinosa, Jose R. and Konstandin, Thomas and Riva, Francesco",
    title = "{Strong Electroweak Phase Transitions in the Standard Model with a Singlet}",
    eprint = "1107.5441",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-PH-TH-2011-171",
    doi = "10.1016/j.nuclphysb.2011.09.010",
    journal = "Nucl. Phys. B",
    volume = "854",
    pages = "592--630",
    year = "2012"
}


@article{Chen:2017qcz,
    author = "Chen, Chien-Yi and Kozaczuk, Jonathan and Lewis, Ian M.",
    title = "{Non-resonant Collider Signatures of a Singlet-Driven Electroweak Phase Transition}",
    eprint = "1704.05844",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "ACFI-T17-07, SLAC-PUB-16951",
    doi = "10.1007/JHEP08(2017)096",
    journal = "JHEP",
    volume = "08",
    pages = "096",
    year = "2017"
}


@article{Ellis:2018mja,
    author = "Ellis, John and Lewicki, Marek and No, Jos\'e Miguel",
    title = "{On the Maximal Strength of a First-Order Electroweak Phase Transition and its Gravitational Wave Signal}",
    eprint = "1809.08242",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KCL-PH-TH/2018-46, CERN-TH/2018-197, IFT-UAM/CSIC-18-94, CERN-TH-2018-197",
    doi = "10.1088/1475-7516/2019/04/003",
    journal = "JCAP",
    volume = "04",
    pages = "003",
    year = "2019"
}




@article{,
    author = "Baldes, Iason and Blasi, Simone and Mariotti, Alberto and Sevrin, Alexander and Turbang, Kevin",
    title = "{Baryogenesis via relativistic bubble expansion}",
    eprint = "2106.15602",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "ULB-TH/21-09",
    month = "6",
    year = "2021"
}
@article{Angelescu:2018dkk,
    author = "Angelescu, Andrei and Huang, Peisi",
    title = "{Multistep Strongly First Order Phase Transitions from New Fermions at the TeV Scale}",
    eprint = "1812.08293",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.99.055023",
    journal = "Phys. Rev. D",
    volume = "99",
    number = "5",
    pages = "055023",
    year = "2019"
}

@article{Hoeche:2020rsg,
    author = {H\"oche, Stefan and Kozaczuk, Jonathan and Long, Andrew J. and Turner, Jessica and Wang, Yikun},
    title = "{Towards an all-orders calculation of the electroweak bubble wall velocity}",
    eprint = "2007.10343",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-20-274-T",
    doi = "10.1088/1475-7516/2021/03/009",
    journal = "JCAP",
    volume = "03",
    pages = "009",
    year = "2021"
}

@article{Barr:1990vd,
    author = "Barr, Stephen M. and Zee, A.",
    title = "{Electric Dipole Moment of the Electron and of the Neutron}",
    reportNumber = "NSF-ITP-90-46",
    doi = "10.1103/PhysRevLett.65.21",
    journal = "Phys. Rev. Lett.",
    volume = "65",
    pages = "21--24",
    year = "1990",
    note = "[Erratum: Phys.Rev.Lett. 65, 2920 (1990)]"
}


@article{Nelson:1991ab,
    author = "Nelson, A. E. and Kaplan, D. B. and Cohen, Andrew G.",
    title = "{Why there is something rather than nothing: Matter from weak interactions}",
    reportNumber = "UCSD-PTH-91-20, BUHEP-91-15",
    doi = "10.1016/0550-3213(92)90440-M",
    journal = "Nucl. Phys. B",
    volume = "373",
    pages = "453--478",
    year = "1992"
}

@article{Bhattacharya:2014a,
    author = "Bhattacharya, Tanmoy and others",
    title = "{QCD Phase Transition with Chiral Quarks and Physical Quark Masses}",
    eprint = "1402.5175",
    archivePrefix = "arXiv",
    primaryClass = "hep-lat",
    reportNumber = "BNL-103837-2014-JA, CU-TP-1205, INT-PUB-14-003, LLNL-JRNL-650194",
    doi = "10.1103/PhysRevLett.113.082001",
    journal = "Phys. Rev. Lett.",
    volume = "113",
    number = "8",
    pages = "082001",
    year = "2014"
}

@article{Carena:1996wj,
    author = "Carena, Marcela and Quiros, M. and Wagner, C. E. M.",
    title = "{Opening the window for electroweak baryogenesis}",
    eprint = "hep-ph/9603420",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-96-30, IEM-FT-126-96",
    doi = "10.1016/0370-2693(96)00475-3",
    journal = "Phys. Lett. B",
    volume = "380",
    pages = "81--91",
    year = "1996"
}

@article{Kajantie:1996mn,
    author = "Kajantie, K. and Laine, M. and Rummukainen, K. and Shaposhnikov, Mikhail E.",
    title = "{Is there a hot electroweak phase transition at m(H) larger or equal to m(W)?}",
    eprint = "hep-ph/9605288",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-96-126, HD-THEP-96-15, IUHET-333",
    doi = "10.1103/PhysRevLett.77.2887",
    journal = "Phys. Rev. Lett.",
    volume = "77",
    pages = "2887--2890",
    year = "1996"
}


@article{Baldes:2020kam,
    author = "Baldes, Iason and Gouttenoire, Yann and Sala, Filippo",
    title = "{String Fragmentation in Supercooled Confinement and Implications for Dark Matter}",
    eprint = "2007.08440",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-20-122",
    doi = "10.1007/JHEP04(2021)278",
    journal = "JHEP",
    volume = "04",
    pages = "278",
    year = "2021"
}


@article{Flanz:1994yx,
    author = "Flanz, Marion and Paschos, Emmanuel A. and Sarkar, Utpal",
    title = "{Baryogenesis from a lepton asymmetric universe}",
    eprint = "hep-ph/9411366",
    archivePrefix = "arXiv",
    reportNumber = "DO-TH-94-15",
    doi = "10.1016/0370-2693(94)01555-Q",
    journal = "Phys. Lett. B",
    volume = "345",
    pages = "248--252",
    year = "1995",
    note = "[Erratum: Phys.Lett.B 384, 487--487 (1996), Erratum: Phys.Lett.B 382, 447--447 (1996)]"
}

@article{Covi:1996wh,
    author = "Covi, Laura and Roulet, Esteban and Vissani, Francesco",
    title = "{CP violating decays in leptogenesis scenarios}",
    eprint = "hep-ph/9605319",
    archivePrefix = "arXiv",
    reportNumber = "SISSA-66-96-EP, IC-96-73",
    doi = "10.1016/0370-2693(96)00817-9",
    journal = "Phys. Lett. B",
    volume = "384",
    pages = "169--174",
    year = "1996"
}

article{Pilaftsis:1997jf,
    author = "Pilaftsis, Apostolos",
    title = "{CP violation and baryogenesis due to heavy Majorana neutrinos}",
    eprint = "hep-ph/9707235",
    archivePrefix = "arXiv",
    reportNumber = "MPI-PHT-97-30",
    doi = "10.1103/PhysRevD.56.5431",
    journal = "Phys. Rev. D",
    volume = "56",
    pages = "5431--5451",
    year = "1997"
}



@article{Azatov:2021ifm,
    author = "Azatov, Aleksandr and Vanvlasselaer, Miguel and Yin, Wen",
    title = "{Dark Matter production from relativistic bubble walls}",
    eprint = "2101.05721",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SISSA 03/2021/FISI",
    doi = "10.1007/JHEP03(2021)288",
    journal = "JHEP",
    volume = "03",
    pages = "288",
    year = "2021"
}


@inproceedings{Riotto:1998bt,
    author = "Riotto, Antonio",
    title = "{Theories of baryogenesis}",
    booktitle = "{ICTP Summer School in High-Energy Physics and Cosmology}",
    eprint = "hep-ph/9807454",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-98-204",
    month = "7",
    year = "1998"
}

BibTeX


@article{Shifman:1979eb,
    author = "Shifman, Mikhail A. and Vainshtein, A. I. and Voloshin, M. B. and Zakharov, Valentin I.",
    title = "{Low-Energy Theorems for Higgs Boson Couplings to Photons}",
    reportNumber = "ITEP-42-1979, ITEP-42",
    journal = "Sov. J. Nucl. Phys.",
    volume = "30",
    pages = "711--716",
    year = "1979"
}

@article{Ellis:1975ap,
    author = "Ellis, John R. and Gaillard, Mary K. and Nanopoulos, Dimitri V.",
    title = "{A Phenomenological Profile of the Higgs Boson}",
    reportNumber = "CERN-TH-2093",
    doi = "10.1016/0550-3213(76)90382-5",
    journal = "Nucl. Phys. B",
    volume = "106",
    pages = "292",
    year = "1976"
}

@article{Liu:1992tn,
    author = "Liu, Bao-Hua and McLerran, Larry D. and Turok, Neil",
    title = "{Bubble nucleation and growth at a baryon number producing electroweak phase transition}",
    reportNumber = "TPI-MINN-92-18-T",
    doi = "10.1103/PhysRevD.46.2668",
    journal = "Phys. Rev. D",
    volume = "46",
    pages = "2668--2688",
    year = "1992"
}


@article{Gisbert:2019ftm,
    author = "Gisbert, Hector and Ruiz Vidal, Joan",
    title = "{Improved bounds on heavy quark electric dipole moments}",
    eprint = "1905.02513",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IFIC/19-24, FTUV/19-0508",
    doi = "10.1103/PhysRevD.101.115010",
    journal = "Phys. Rev. D",
    volume = "101",
    number = "11",
    pages = "115010",
    year = "2020"
}


@book{Akhiezer:1986yqm,
    author = "Akhiezer, A.I. and Berestetskii, V.B.",
    title = "{Quantum electrodynamics}",
    reportNumber = "AEC-TR-2876",
    month = "9",
    year = "1986",
    publisher=  "Interscience Publishers",
    isbn="0470018488",
    address= "New York"
    
}


@article{Altarelli:1977zs,
    author = "Altarelli, Guido and Parisi, G.",
    title = "{Asymptotic Freedom in Parton Language}",
    reportNumber = "LPTENS-77-6",
    doi = "10.1016/0550-3213(77)90384-4",
    journal = "Nucl. Phys. B",
    volume = "126",
    pages = "298--318",
    year = "1977"
}


@article{Dokshitzer:1977sg,
    author = "Dokshitzer, Yuri L.",
    title = "{Calculation of the Structure Functions for Deep Inelastic Scattering and e+ e- Annihilation by Perturbation Theory in Quantum Chromodynamics.}",
    journal = "Sov. Phys. JETP",
    volume = "46",
    pages = "641--653",
    year = "1977"
}




@article{Azatov:2019png,
    author = "Azatov, Aleksandr and Barducci, Daniele and Sgarlata, Francesco",
    title = "{Gravitational traces of broken gauge symmetries}",
    eprint = "1910.01124",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SISSA 28/2019/FISI",
    doi = "10.1088/1475-7516/2020/07/027",
    journal = "JCAP",
    volume = "07",
    pages = "027",
    year = "2020"
}




@article{Gribov:1972rt,
    author = "Gribov, V.N. and Lipatov, L.N.",
    title = "{e+ e- pair annihilation and deep inelastic e p scattering in perturbation theory}",
    journal = "Sov. J. Nucl. Phys.",
    volume = "15",
    pages = "675--684",
    year = "1972"
}


@book{Peskin:1995ev,
    author = "Peskin, Michael E. and Schroeder, Daniel V.",
    title = "{An Introduction to quantum field theory}",
    isbn = "978-0-201-50397-5",
    publisher = "Addison-Wesley",
    address = "Reading, USA",
    year = "1995"
}



@book{Berestetsky:1982aq,
    author = "Berestetskii, V.B. and Lifshitz, E.M. and Pitaevskii, L.P.",
    title = "{QUANTUM ELECTRODYNAMICS}",
    isbn = "978-0-7506-3371-0",
    publisher = "Pergamon Press",
    address = "Oxford",
    series = "Course of Theoretical Physics",
    volume = "4",
    year = "1982"
}






@article{Arnold:1993wc,
    author = "Arnold, Peter Brockway",
    title = "{One loop fluctuation - dissipation formula for bubble wall velocity}",
    eprint = "hep-ph/9302258",
    archivePrefix = "arXiv",
    reportNumber = "UW-PT-93-2",
    doi = "10.1103/PhysRevD.48.1539",
    journal = "Phys. Rev. D",
    volume = "48",
    pages = "1539--1545",
    year = "1993"
}



@article{Grasso:2000wj,
    author = "Grasso, Dario and Rubinstein, Hector R.",
    title = "{Magnetic fields in the early universe}",
    eprint = "astro-ph/0009061",
    archivePrefix = "arXiv",
    reportNumber = "DFPD-00-TH-35",
    doi = "10.1016/S0370-1573(00)00110-1",
    journal = "Phys. Rept.",
    volume = "348",
    pages = "163--266",
    year = "2001"
}


@article{Kuzmin:1985mm,
    author = "Kuzmin, V.A. and Rubakov, V.A. and Shaposhnikov, M.E.",
    title = "{On the Anomalous Electroweak Baryon Number Nonconservation in the Early Universe}",
    reportNumber = "IC/85/8",
    doi = "10.1016/0370-2693(85)91028-7",
    journal = "Phys. Lett. B",
    volume = "155",
    pages = "36",
    year = "1985"
}



@article{Shaposhnikov:1986jp,
    author = "Shaposhnikov, M.E.",
    title = "{Possible Appearance of the Baryon Asymmetry of the Universe in an Electroweak Theory}",
    journal = "JETP Lett.",
    volume = "44",
    pages = "465--468",
    year = "1986"
}



@article{Konstandin:2013caa,
    author = "Konstandin, Thomas",
    title = "{Quantum Transport and Electroweak Baryogenesis}",
    eprint = "1302.6713",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-13-036",
    doi = "10.3367/UFNe.0183.201308a.0785",
    journal = "Phys. Usp.",
    volume = "56",
    pages = "747--771",
    year = "2013"
}




@article{fermi:24,
    author = "Fermi , Enrico",
    title = "{Uber die Theorie des Stoßes zwischen Atomen und elektrisch geladenen Teilchen}",
      journal        = "Zeitschrift fur Physik",
      volume         = "29",
      year           = "1924",
      number         = "1",
      pages          = "315--327",
      doi            = "10.1007/BF03184853"
     }

@article{landau:34,
    author = "Landau, Lev and  Lifshitz, Evgeni",
    title = " ",
      journal        = "Phys.Z.Sowjetunion",
      volume         = "6",
      year           = "1934",
      number         = "1",
      pages          = "612",
      doi            = ""
     }     
     

@article{vonWeizsacker:1934nji,
    author = "von Weizsacker, C.F.",
    title = "{Radiation emitted in collisions of very fast electrons}",
    doi = "10.1007/BF01333110",
    journal = "Z. Phys.",
    volume = "88",
    pages = "612--625",
    year = "1934"
}

@article{Williams:1934ad,
    author = "Williams, E.J.",
    title = "{Nature of the high-energy particles of penetrating radiation and status of ionization and radiation formulae}",
    doi = "10.1103/PhysRev.45.729",
    journal = "Phys. Rev.",
    volume = "45",
    pages = "729--730",
    year = "1934"
}


     
     

@article{Mancha:2020fzw,
    author = "Barroso Mancha, Marc and Prokopec, Tomislav and Swiezewska, Bogumila",
    title = "{Field theoretic derivation of bubble wall force}",
    eprint = "2005.10875",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "5",
    year = "2020"
}



@article{Hansen:2017pwe,
      author         = "Hansen, Frederik F. and Janowski, Tadeusz and Langable,
                        Kasper and Mann, Robert B. and Sannino, Francesco and
                        Steele, Tom G. and Wang, Zhi-Wei",
      title          = "{Phase structure of complete asymptotically free
                        SU($N_c$) theories with quarks and scalar quarks}",
      journal        = "Phys. Rev.",
      volume         = "D97",
      year           = "2018",
      number         = "6",
      pages          = "065014",
      doi            = "10.1103/PhysRevD.97.065014",
      eprint         = "1706.06402",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CP3-ORIGINS-2017-022, CERN-TH-2017-133",
      SLACcitation   = "%%CITATION = ARXIV:1706.06402;%%"
}


@article{Bruggisser:2018mus,
    author = "Bruggisser, Sebastian and Von Harling, Benedict and Matsedonskyi, Oleksii and Servant, Géraldine",
    title = "{Baryon Asymmetry from a Composite Higgs Boson}",
    eprint = "1803.08546",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-18-029",
    doi = "10.1103/PhysRevLett.121.131801",
    journal = "Phys. Rev. Lett.",
    volume = "121",
    number = "13",
    pages = "131801",
    year = "2018"
}



@article{Bruggisser:2018mrt,
    author = "Bruggisser, Sebastian and Von Harling, Benedict and Matsedonskyi, Oleksii and Servant, Géraldine",
    title = "{Electroweak Phase Transition and Baryogenesis in Composite Higgs Models}",
    eprint = "1804.07314",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-17-229",
    doi = "10.1007/JHEP12(2018)099",
    journal = "JHEP",
    volume = "12",
    pages = "099",
    year = "2018"
}



@article{DelleRose:2019pgi,
    author = "Delle Rose, Luigi and Panico, Giuliano and Redi, Michele and Tesi, Andrea",
    title = "{Gravitational Waves from Supercool Axions}",
    eprint = "1912.06139",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP04(2020)025",
    journal = "JHEP",
    volume = "04",
    pages = "025",
    year = "2020"
}



@article{Antipin:2012kc,
      author         = "Antipin, Oleg and Di Chiara, Stefano and Mojaza, Matin
                        and Molgaard, Esben and Sannino, Francesco",
      title          = "{A Perturbative Realization of Miransky Scaling}",
      journal        = "Phys. Rev.",
      volume         = "D86",
      year           = "2012",
      pages          = "085009",
      doi            = "10.1103/PhysRevD.86.085009",
      eprint         = "1205.6157",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CP3-ORIGINS-2012-15, DIAS-ORIGINS-2012-16",
      SLACcitation   = "%%CITATION = ARXIV:1205.6157;%%"
}


@article{Miransky:1984ef,
      author         = "Miransky, V. A.",
      title          = "{Dynamics of Spontaneous Chiral Symmetry Breaking and
                        Continuum Limit in Quantum Electrodynamics}",
      journal        = "Nuovo Cim.",
      volume         = "A90",
      year           = "1985",
      pages          = "149-170",
      doi            = "10.1007/BF02724229",
      reportNumber   = "ITF-84-152E",
      SLACcitation   = "%%CITATION = NUCIA,A90,149;%%"
}


@article{Coradeschi:2013gda,
      author         = "Coradeschi, Francesco and Lodone, Paolo and Pappadopulo,
                        Duccio and Rattazzi, Riccardo and Vitale, Lorenzo",
      title          = "{A naturally light dilaton}",
      journal        = "JHEP",
      volume         = "11",
      year           = "2013",
      pages          = "057",
      doi            = "10.1007/JHEP11(2013)057",
      eprint         = "1306.4601",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1306.4601;%%"
}

@article{Bunk:2017fic,
      author         = "Bunk, Don and Hubisz, Jay and Jain, Bithika",
      title          = "{A Perturbative RS I Cosmological Phase Transition}",
      journal        = "Eur. Phys. J.",
      volume         = "C78",
      year           = "2018",
      number         = "1",
      pages          = "78",
      doi            = "10.1140/epjc/s10052-018-5529-2",
      eprint         = "1705.00001",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1705.00001;%%"
}



@article{Appelquist:1986an,
      author         = "Appelquist, Thomas W. and Karabali, Dimitra and
                        Wijewardhana, L. C. R.",
      title          = "{Chiral Hierarchies and the Flavor Changing Neutral
                        Current Problem in Technicolor}",
      journal        = "Phys. Rev. Lett.",
      volume         = "57",
      year           = "1986",
      pages          = "957",
      doi            = "10.1103/PhysRevLett.57.957",
      reportNumber   = "YTP-86/11",
      SLACcitation   = "%%CITATION = PRLTA,57,957;%%"
}


@article{Luty:2004ye,
      author         = "Luty, Markus A. and Okui, Takemichi",
      title          = "{Conformal technicolor}",
      journal        = "JHEP",
      volume         = "09",
      year           = "2006",
      pages          = "070",
      doi            = "10.1088/1126-6708/2006/09/070",
      eprint         = "hep-ph/0409274",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "BUHEP-04-12, UMD-PP-05-017",
      SLACcitation   = "%%CITATION = HEP-PH/0409274;%%"
}



@article{Hill:2002ap,
      author         = "Hill, Christopher T. and Simmons, Elizabeth H.",
      title          = "{Strong Dynamics and Electroweak Symmetry Breaking}",
      journal        = "Phys. Rept.",
      volume         = "381",
      year           = "2003",
      pages          = "235-402",
      doi            = "10.1016/S0370-1573(03)00140-6",
      note           = "[Erratum: Phys. Rept.390,553(2004)]",
      eprint         = "hep-ph/0203079",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-02-045-T, BUHEP-01-09",
      SLACcitation   = "%%CITATION = HEP-PH/0203079;%%"
}


@article{Yamawaki:1985zg,
      author         = "Yamawaki, Koichi and Bando, Masako and Matumoto, Ken-iti",
      title          = "{Scale Invariant Technicolor Model and a Technidilaton}",
      journal        = "Phys. Rev. Lett.",
      volume         = "56",
      year           = "1986",
      pages          = "1335",
      doi            = "10.1103/PhysRevLett.56.1335",
      reportNumber   = "DPNU-85-47",
      SLACcitation   = "%%CITATION = PRLTA,56,1335;%%"
}


@article{Holdom:1981rm,
      author         = "Holdom, Bob",
      title          = "{Raising the Sideways Scale}",
      journal        = "Phys. Rev.",
      volume         = "D24",
      year           = "1981",
      pages          = "1441",
      doi            = "10.1103/PhysRevD.24.1441",
      reportNumber   = "HUTP-81-A025",
      SLACcitation   = "%%CITATION = PHRVA,D24,1441;%%"
}


@article{Caprini:2019egz,
      author         = "Caprini, Chiara and others",
      title          = "{Detecting gravitational waves from cosmological phase
                        transitions with LISA: an update}",
      year           = "2019",
      eprint         = "1910.13125",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "DESY-19-159, IPPP/19/27, HIP-2019-14/TH, MITP/19-066,
                        IFT-UAM/CSIC-19-139",
      SLACcitation   = "%%CITATION = ARXIV:1910.13125;%%"
}



@article{Dine:1992wr,
      author         = "Dine, Michael and Leigh, Robert G. and Huet, Patrick Y.
                        and Linde, Andrei D. and Linde, Dmitri A.",
      title          = "{Towards the theory of the electroweak phase transition}",
      journal        = "Phys. Rev.",
      volume         = "D46",
      year           = "1992",
      pages          = "550-571",
      doi            = "10.1103/PhysRevD.46.550",
      eprint         = "hep-ph/9203203",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SLAC-PUB-5741, SCIPP-92-07, SU-ITP-92-7",
      SLACcitation   = "%%CITATION = HEP-PH/9203203;%%"
}


@article{Comelli:1996vm,
      author         = "Comelli, D. and Espinosa, J. R.",
      title          = "{Bosonic thermal masses in supersymmetry}",
      journal        = "Phys. Rev.",
      volume         = "D55",
      year           = "1997",
      pages          = "6253-6263",
      doi            = "10.1103/PhysRevD.55.6253",
      eprint         = "hep-ph/9606438",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-96-114, FTUV-96-37, IFIC-96-45, IEM-FT-134-96",
      SLACcitation   = "%%CITATION = HEP-PH/9606438;%%"
}


@article{Bellazzini:2014yua,
      author         = "Bellazzini, Brando and Csaki, Csaba and Serra, Javi",
      title          = "{Composite Higgses}",
      journal        = "Eur. Phys. J.",
      volume         = "C74",
      year           = "2014",
      number         = "5",
      pages          = "2766",
      doi            = "10.1140/epjc/s10052-014-2766-x",
      eprint         = "1401.2457",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1401.2457;%%"
}



@article{Goldberger:1999uk,
      author         = "Goldberger, Walter D. and Wise, Mark B.",
      title          = "{Modulus stabilization with bulk fields}",
      journal        = "Phys. Rev. Lett.",
      volume         = "83",
      year           = "1999",
      pages          = "4922-4925",
      doi            = "10.1103/PhysRevLett.83.4922",
      eprint         = "hep-ph/9907447",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CALT-68-2232",
      SLACcitation   = "%%CITATION = HEP-PH/9907447;%%"
}



@article{Randall:1999ee,
      author         = "Randall, Lisa and Sundrum, Raman",
      title          = "{A Large mass hierarchy from a small extra dimension}",
      journal        = "Phys. Rev. Lett.",
      volume         = "83",
      year           = "1999",
      pages          = "3370-3373",
      doi            = "10.1103/PhysRevLett.83.3370",
      eprint         = "hep-ph/9905221",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MIT-CTP-2860, PUPT-1860, BUHEP-99-9",
      SLACcitation   = "%%CITATION = HEP-PH/9905221;%%"
}



@article{Caswell:1974gg,
      author         = "Caswell, William E.",
      title          = "{Asymptotic Behavior of Nonabelian Gauge Theories to Two
                        Loop Order}",
      journal        = "Phys. Rev. Lett.",
      volume         = "33",
      year           = "1974",
      pages          = "244",
      doi            = "10.1103/PhysRevLett.33.244",
      reportNumber   = "PRINT-74-1058 (PRINCETON)",
      SLACcitation   = "%%CITATION = PRLTA,33,244;%%"
}


@article{Banks:1981nn,
      author         = "Banks, Tom and Zaks, A.",
      title          = "{On the Phase Structure of Vector-Like Gauge Theories
                        with Massless Fermions}",
      journal        = "Nucl. Phys.",
      volume         = "B196",
      year           = "1982",
      pages          = "189-204",
      doi            = "10.1016/0550-3213(82)90035-9",
      reportNumber   = "TAUP-944-81",
      SLACcitation   = "%%CITATION = NUPHA,B196,189;%%"
}



@article{Benini:2019dfy,
      author         = "Benini, Francesco and Iossa, Cristoforo and Serone,
                        Marco",
      title          = "{Conformality Loss, Walking, and 4D Complex Conformal
                        Field Theories at Weak Coupling}",
      journal        = "Phys. Rev. Lett.",
      volume         = "124",
      year           = "2020",
      number         = "5",
      pages          = "051602",
      doi            = "10.1103/PhysRevLett.124.051602",
      eprint         = "1908.04325",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "SISSA 21/2019/FISI",
      SLACcitation   = "%%CITATION = ARXIV:1908.04325;%%"
}



@article{Randall:2006py,
      author         = "Randall, Lisa and Servant, Geraldine",
      title          = "{Gravitational waves from warped spacetime}",
      journal        = "JHEP",
      volume         = "05",
      year           = "2007",
      pages          = "054",
      doi            = "10.1088/1126-6708/2007/05/054",
      eprint         = "hep-ph/0607158",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-PH-TH-2006-133",
      SLACcitation   = "%%CITATION = HEP-PH/0607158;%%"
}






@article{Agashe:2019lhy,
      author         = "Agashe, Kaustubh and Du, Peizhi and Ekhterachian, Majid
                        and Kumar, Soubhik and Sundrum, Raman",
      title          = "{Cosmological Phase Transition of Spontaneous
                        Confinement}",
      year           = "2019",
      eprint         = "1910.06238",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UMD-PP-019-05, YITP-SB-19-32",
      SLACcitation   = "%%CITATION = ARXIV:1910.06238;%%"
}


@article{Gorbenko:2018ncu,
      author         = "Gorbenko, Victor and Rychkov, Slava and Zan, Bernardo",
      title          = "{Walking, Weak first-order transitions, and Complex
                        CFTs}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2018",
      pages          = "108",
      doi            = "10.1007/JHEP10(2018)108",
      eprint         = "1807.11512",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1807.11512;%%"
}



@article{Kaplan:2009kr,
      author         = "Kaplan, David B. and Lee, Jong-Wan and Son, Dam T. and
                        Stephanov, Mikhail A.",
      title          = "{Conformality Lost}",
      journal        = "Phys. Rev.",
      volume         = "D80",
      year           = "2009",
      pages          = "125005",
      doi            = "10.1103/PhysRevD.80.125005",
      eprint         = "0905.4752",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "INT-PUB-09-020",
      SLACcitation   = "%%CITATION = ARXIV:0905.4752;%%"
}



@article{Rattazzi:2008pe,
      author         = "Rattazzi, Riccardo and Rychkov, Vyacheslav S. and Tonni,
                        Erik and Vichi, Alessandro",
      title          = "{Bounding scalar operator dimensions in 4D CFT}",
      journal        = "JHEP",
      volume         = "12",
      year           = "2008",
      pages          = "031",
      doi            = "10.1088/1126-6708/2008/12/031",
      eprint         = "0807.0004",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:0807.0004;%%"
}



@inproceedings{Contino:2010rs,
      author         = "Contino, Roberto",
      title          = "{The Higgs as a Composite Nambu-Goldstone Boson}",
      booktitle      = "{Physics of the large and the small, TASI 09, proceedings
                        of the Theoretical Advanced Study Institute in Elementary
                        Particle Physics, Boulder, Colorado, USA, 1-26 June 2009}",
      year           = "2011",
      pages          = "235-306",
      doi            = "10.1142/9789814327183_0005",
      eprint         = "1005.4269",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1005.4269;%%"
}



@article{Alanne:2019bsm,
      author         = "Alanne, Tommi and Hugle, Thomas and Platscher, Moritz and
                        Schmitz, Kai",
      title          = "{A fresh look at the gravitational-wave signal from
                        cosmological phase transitions}",
      year           = "2019",
      eprint         = "1909.11356",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1909.11356;%%"
}

@article{Moore:1995ua,
      author         = "Moore, Guy D. and Prokopec, Tomislav",
      title          = "{Bubble wall velocity in a first order electroweak phase
                        transition}",
      journal        = "Phys. Rev. Lett.",
      volume         = "75",
      year           = "1995",
      pages          = "777-780",
      doi            = "10.1103/PhysRevLett.75.777",
      eprint         = "hep-ph/9503296",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "PUPT-1531, LANCASTER-TH-9503, PUP-TH-1531-(1995),
                        LANCASTER-TH-9503-(1995)",
      SLACcitation   = "%%CITATION = HEP-PH/9503296;%%"
}
@article{Moore:1995si,
      author         = "Moore, Guy D. and Prokopec, Tomislav",
      title          = "{How fast can the wall move? A Study of the electroweak
                        phase transition dynamics}",
      journal        = "Phys. Rev.",
      volume         = "D52",
      year           = "1995",
      pages          = "7182-7204",
      doi            = "10.1103/PhysRevD.52.7182",
      eprint         = "hep-ph/9506475",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "PUPT-1544, PUP-TH-1544, LANCS-TH-9517",
      SLACcitation   = "%%CITATION = HEP-PH/9506475;%%"
}

@article{Dorsch:2018pat,
      author         = "Dorsch, Glauber C. and Huber, Stephan J. and Konstandin,
                        Thomas",
      title          = "{Bubble wall velocities in the Standard Model and
                        beyond}",
      journal        = "JCAP",
      volume         = "1812",
      year           = "2018",
      number         = "12",
      pages          = "034",
      doi            = "10.1088/1475-7516/2018/12/034",
      eprint         = "1809.04907",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY 18-162, DESY-18-162",
      SLACcitation   = "%%CITATION = ARXIV:1809.04907;%%"
}



@article{Hiramatsu:2013qaa,
    author = "Hiramatsu, Takashi and Kawasaki, Masahiro and Saikawa, Ken'ichi",
    title = "{On the estimation of gravitational wave spectrum from cosmic domain walls}",
    eprint = "1309.5001",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "ICRR-REPORT-659-2013-8, IPMU13-0182, YITP-13-87",
    doi = "10.1088/1475-7516/2014/02/031",
    journal = "JCAP",
    volume = "02",
    pages = "031",
    year = "2014"
}



@article{Espinosa:2010hh,
      author         = "Espinosa, Jose R. and Konstandin, Thomas and No, Jose M.
                        and Servant, Geraldine",
      title          = "{Energy Budget of Cosmological First-order Phase
                        Transitions}",
      journal        = "JCAP",
      volume         = "1006",
      year           = "2010",
      pages          = "028",
      doi            = "10.1088/1475-7516/2010/06/028",
      eprint         = "1004.4187",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-PH-TH-2010-027",
      SLACcitation   = "%%CITATION = ARXIV:1004.4187;%%"
}

@article{Bodeker:2009qy,
      author         = "Bodeker, Dietrich and Moore, Guy D.",
      title          = "{Can electroweak bubble walls run away?}",
      journal        = "JCAP",
      volume         = "0905",
      year           = "2009",
      pages          = "009",
      doi            = "10.1088/1475-7516/2009/05/009",
      eprint         = "0903.4099",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0903.4099;%%"
}


@article{Bodeker:2017cim,
      author         = "Bodeker, Dietrich and Moore, Guy D.",
      title          = "{Electroweak Bubble Wall Speed Limit}",
      journal        = "JCAP",
      volume         = "1705",
      year           = "2017",
      number         = "05",
      pages          = "025",
      doi            = "10.1088/1475-7516/2017/05/025",
      eprint         = "1703.08215",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1703.08215;%%"
}


@article{Curtin:2016urg,
      author         = "Curtin, David and Meade, Patrick and Ramani,
                        Harikrishnan",
      title          = "{Thermal Resummation and Phase Transitions}",
      journal        = "Eur. Phys. J.",
      volume         = "C78",
      year           = "2018",
      number         = "9",
      pages          = "787",
      doi            = "10.1140/epjc/s10052-018-6268-0",
      eprint         = "1612.00466",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "YITP-2016-48",
      SLACcitation   = "%%CITATION = ARXIV:1612.00466;%%"
}

@article{Baratella:2018pxi,
      author         = "Baratella, Pietro and Pomarol, Alex and Rompineve,
                        Fabrizio",
      title          = "{The Supercooled Universe}",
      journal        = "JHEP",
      volume         = "03",
      year           = "2019",
      pages          = "100",
      doi            = "10.1007/JHEP03(2019)100",
      eprint         = "1812.06996",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1812.06996;%%"
}

@article{Caprini:2015zlo,
      author         = "Caprini, Chiara and others",
      title          = "{Science with the space-based interferometer eLISA. II:
                        Gravitational waves from cosmological phase transitions}",
      journal        = "JCAP",
      volume         = "1604",
      year           = "2016",
      number         = "04",
      pages          = "001",
      doi            = "10.1088/1475-7516/2016/04/001",
      eprint         = "1512.06239",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "DESY-15-246",
      SLACcitation   = "%%CITATION = ARXIV:1512.06239;%%"
}

@article{Ellis:2019oqb,
      author         = "Ellis, John and Lewicki, Marek and No, Jos� Miguel and
                        Vaskonen, Ville",
      title          = "{Gravitational wave energy budget in strongly supercooled
                        phase transitions}",
      journal        = "JCAP",
      volume         = "1906",
      year           = "2019",
      number         = "06",
      pages          = "024",
      doi            = "10.1088/1475-7516/2019/06/024",
      eprint         = "1903.09642",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KCL-PH-TH/2019-32, CERN-TH-2019-032, IFT-UAM/CSIC-19-32",
      SLACcitation   = "%%CITATION = ARXIV:1903.09642;%%"
}

@article{Caprini:2007xq,
      author         = "Caprini, Chiara and Durrer, Ruth and Servant, Geraldine",
      title          = "{Gravitational wave generation from bubble collisions in
                        first-order phase transitions: An analytic approach}",
      journal        = "Phys. Rev.",
      volume         = "D77",
      year           = "2008",
      pages          = "124015",
      doi            = "10.1103/PhysRevD.77.124015",
      eprint         = "0711.2593",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "CERN-PH-TH-2007-206, SACLAY-T07-142",
      SLACcitation   = "%%CITATION = ARXIV:0711.2593;%%"
}




@article{vonHarling:2017yew,
      author         = "von Harling, Benedict and Servant, Geraldine",
      title          = "{QCD-induced Electroweak Phase Transition}",
      journal        = "JHEP",
      volume         = "01",
      year           = "2018",
      pages          = "159",
      doi            = "10.1007/JHEP01(2018)159",
      eprint         = "1711.11554",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-17-056",
      SLACcitation   = "%%CITATION = ARXIV:1711.11554;%%"
}

@article{Hindmarsh:2015qta,
      author         = "Hindmarsh, Mark and Huber, Stephan J. and Rummukainen,
                        Kari and Weir, David J.",
      title          = "{Numerical simulations of acoustically generated
                        gravitational waves at a first order phase transition}",
      journal        = "Phys. Rev.",
      volume         = "D92",
      year           = "2015",
      number         = "12",
      pages          = "123009",
      doi            = "10.1103/PhysRevD.92.123009",
      eprint         = "1504.03291",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "HIP-2015-13-TH",
      SLACcitation   = "%%CITATION = ARXIV:1504.03291;%%"
}


@article{Hindmarsh:2017gnf,
      author         = "Hindmarsh, Mark and Huber, Stephan J. and Rummukainen,
                        Kari and Weir, David J.",
      title          = "{Shape of the acoustic gravitational wave power spectrum
                        from a first order phase transition}",
      journal        = "Phys. Rev.",
      volume         = "D96",
      year           = "2017",
      number         = "10",
      pages          = "103520",
      doi            = "10.1103/PhysRevD.96.103520",
      eprint         = "1704.05871",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "HIP-2017-02-TH",
      SLACcitation   = "%%CITATION = ARXIV:1704.05871;%%"
}


@article{Cutting:2018tjt,
      author         = "Cutting, Daniel and Hindmarsh, Mark and Weir, David J.",
      title          = "{Gravitational waves from vacuum first-order phase
                        transitions: from the envelope to the lattice}",
      journal        = "Phys. Rev.",
      volume         = "D97",
      year           = "2018",
      number         = "12",
      pages          = "123513",
      doi            = "10.1103/PhysRevD.97.123513",
      eprint         = "1802.05712",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "HIP-2018-4-TH",
      SLACcitation   = "%%CITATION = ARXIV:1802.05712;%%"
}



@article{Fairbairn:2019xog,
      author         = "Fairbairn, Malcolm and Hardy, Edward and Wickens,
                        Alastair",
      title          = "{Hearing without seeing: gravitational waves from hot and
                        cold hidden sectors}",
      journal        = "JHEP",
      volume         = "07",
      year           = "2019",
      pages          = "044",
      doi            = "10.1007/JHEP07(2019)044",
      eprint         = "1901.11038",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KCL-PH-TH/2019-12, KCL-PH-TH/2019-12",
      SLACcitation   = "%%CITATION = ARXIV:1901.11038;%%"
}

@phdthesis{Weinberg:1973am,
      author         = "Weinberg, Erick J.",
      title          = "{Radiative corrections as the origin of spontaneous
                        symmetry breaking}",
      school         = "Harvard U.",
      year           = "1973",
      eprint         = "hep-th/0507214",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/0507214;%%"
}

@article{Coleman:1977py,
      author         = "Coleman, Sidney R.",
      title          = "{The Fate of the False Vacuum. 1. Semiclassical Theory}",
      journal        = "Phys. Rev.",
      volume         = "D15",
      year           = "1977",
      pages          = "2929-2936",
      doi            = "10.1103/PhysRevD.15.2929, 10.1103/PhysRevD.16.1248",
      note           = "[Erratum: Phys. Rev.D16,1248(1977)]",
      reportNumber   = "HUTP-77-A004",
      SLACcitation   = "%%CITATION = PHRVA,D15,2929;%%"
}



@article{Breitbach:2018ddu,
      author         = "Breitbach, Moritz and Kopp, Joachim and Madge, Eric and
                        Opferkuch, Toby and Schwaller, Pedro",
      title          = "{Dark, Cold, and Noisy: Constraining Secluded Hidden
                        Sectors with Gravitational Waves}",
      journal        = "JCAP",
      volume         = "1907",
      year           = "2019",
      number         = "07",
      pages          = "007",
      doi            = "10.1088/1475-7516/2019/07/007",
      eprint         = "1811.11175",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-TH-2018-255, MITP/18-115",
      SLACcitation   = "%%CITATION = ARXIV:1811.11175;%%"
}


@article{Wainwright:2011kj,
      author         = "Wainwright, Carroll L.",
      title          = "{CosmoTransitions: Computing Cosmological Phase
                        Transition Temperatures and Bubble Profiles with Multiple
                        Fields}",
      journal        = "Comput. Phys. Commun.",
      volume         = "183",
      year           = "2012",
      pages          = "2006-2013",
      doi            = "10.1016/j.cpc.2012.04.004",
      eprint         = "1109.4189",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1109.4189;%%"
}

@article{Sakharov:1967dj,
      author         = "Sakharov, A. D.",
      title          = "{Violation of CP Invariance, C asymmetry, and baryon
                        asymmetry of the universe}",
      journal        = "Pisma Zh. Eksp. Teor. Fiz.",
      volume         = "5",
      year           = "1967",
      pages          = "32-35",
      doi            = "10.1070/PU1991v034n05ABEH002497",
      note           = "[Usp. Fiz. Nauk161,no.5,61(1991)]",
      SLACcitation   = "%%CITATION = ZFPRA,5,32;%%"
}

@article{Abbott:2016blz,
      author         = "Abbott, B. P. and others",
      title          = "{Observation of Gravitational Waves from a Binary Black
                        Hole Merger}",
      collaboration  = "LIGO Scientific, Virgo",
      journal        = "Phys. Rev. Lett.",
      volume         = "116",
      year           = "2016",
      number         = "6",
      pages          = "061102",
      doi            = "10.1103/PhysRevLett.116.061102",
      eprint         = "1602.03837",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      reportNumber   = "LIGO-P150914",
      SLACcitation   = "%%CITATION = ARXIV:1602.03837;%%"
}

@article{GBM:2017lvd,
      author         = "Abbott, B. P. and others",
      title          = "{Multi-messenger Observations of a Binary Neutron Star
                        Merger}",
      collaboration  = "LIGO Scientific, Virgo, Fermi GBM, INTEGRAL, IceCube,
                        AstroSat Cadmium Zinc Telluride Imager Team, IPN,
                        Insight-Hxmt, ANTARES, Swift, AGILE Team, 1M2H Team, Dark
                        Energy Camera GW-EM, DES, DLT40, GRAWITA, Fermi-LAT, ATCA,
                        ASKAP, Las Cumbres Observatory Group, OzGrav, DWF (Deeper
                        Wider Faster Program), AST3, CAASTRO, VINROUGE, MASTER,
                        J-GEM, GROWTH, JAGWAR, CaltechNRAO, TTU-NRAO, NuSTAR,
                        Pan-STARRS, MAXI Team, TZAC Consortium, KU, Nordic Optical
                        Telescope, ePESSTO, GROND, Texas Tech University, SALT
                        Group, TOROS, BOOTES, MWA, CALET, IKI-GW Follow-up,
                        H.E.S.S., LOFAR, LWA, HAWC, Pierre Auger, ALMA, Euro VLBI
                        Team, Pi of Sky, Chandra Team at McGill University, DFN,
                        ATLAS Telescopes, High Time Resolution Universe Survey,
                        RIMAS, RATIR, SKA South Africa/MeerKAT",
      journal        = "Astrophys. J.",
      volume         = "848",
      year           = "2017",
      number         = "2",
      pages          = "L12",
      doi            = "10.3847/2041-8213/aa91c9",
      eprint         = "1710.05833",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      reportNumber   = "LIGO-P1700294, VIR-0802A-17, FERMILAB-PUB-17-478-A-AE-CD",
      SLACcitation   = "%%CITATION = ARXIV:1710.05833;%%"
}

@article{Witten:1984rs,
      author         = "Witten, Edward",
      title          = "{Cosmic Separation of Phases}",
      journal        = "Phys. Rev.",
      volume         = "D30",
      year           = "1984",
      pages          = "272-285",
      doi            = "10.1103/PhysRevD.30.272",
      reportNumber   = "PRINT-84-0400 (IAS,PRINCETON)",
      SLACcitation   = "%%CITATION = PHRVA,D30,272;%%"
}

@article{Thrane:2013oya,
      author         = "Thrane, Eric and Romano, Joseph D.",
      title          = "{Sensitivity curves for searches for gravitational-wave
                        backgrounds}",
      journal        = "Phys. Rev.",
      volume         = "D88",
      year           = "2013",
      number         = "12",
      pages          = "124032",
      doi            = "10.1103/PhysRevD.88.124032",
      eprint         = "1310.5300",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1310.5300;%%"
}

@article{TheLIGOScientific:2014jea,
      author         = "Aasi, J. and others",
      title          = "{Advanced LIGO}",
      collaboration  = "LIGO Scientific",
      journal        = "Class. Quant. Grav.",
      volume         = "32",
      year           = "2015",
      pages          = "074001",
      doi            = "10.1088/0264-9381/32/7/074001",
      eprint         = "1411.4547",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = ARXIV:1411.4547;%%"
}

@article{Aasi:2013wya,
      author         = "Abbott, B. P. and others",
      title          = "{Prospects for Observing and Localizing
                        Gravitational-Wave Transients with Advanced LIGO, Advanced
                        Virgo and KAGRA}",
      collaboration  = "KAGRA, LIGO Scientific, VIRGO",
      journal        = "Living Rev. Rel.",
      volume         = "21",
      year           = "2018",
      number         = "1",
      pages          = "3",
      doi            = "10.1007/s41114-018-0012-9, 10.1007/lrr-2016-1",
      eprint         = "1304.0670",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      reportNumber   = "LIGO-P1200087, VIR-0288A-12",
      SLACcitation   = "%%CITATION = ARXIV:1304.0670;%%"
}

@article{Graham:2017pmn,
      author         = "Graham, Peter W. and Hogan, Jason M. and Kasevich, Mark
                        A. and Rajendran, Surjeet and Romani, Roger W.",
      title          = "{Mid-band gravitational wave detection with precision
                        atomic sensors}",
      collaboration  = "MAGIS",
      year           = "2017",
      eprint         = "1711.02225",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1711.02225;%%"
}

@article{Cornish:2018dyw,
      author         = "Robson, Travis and Cornish, Neil J. and Liug, Chang",
      title          = "{The construction and use of LISA sensitivity curves}",
      journal        = "Class. Quant. Grav.",
      volume         = "36",
      year           = "2019",
      number         = "10",
      pages          = "105011",
      doi            = "10.1088/1361-6382/ab1101",
      eprint         = "1803.01944",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1803.01944;%%"
}
@article{Yagi:2011yu,
      author         = "Yagi, Kent and Tanahashi, Norihiro and Tanaka, Takahiro",
      title          = "{Probing the size of extra dimension with gravitational
                        wave astronomy}",
      journal        = "Phys. Rev.",
      volume         = "D83",
      year           = "2011",
      pages          = "084036",
      doi            = "10.1103/PhysRevD.83.084036",
      eprint         = "1101.4997",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      reportNumber   = "KUNS-2319, YITP-11-11",
      SLACcitation   = "%%CITATION = ARXIV:1101.4997;%%"
}
@article{PhysRevD.80.104009,
  title = {Ultrahigh precision cosmology from gravitational waves},
  author = {Cutler, Curt and Holz, Daniel E.},
  journal = {Phys. Rev. D},
  volume = {80},
  issue = {10},
  pages = {104009},
  numpages = {15},
  year = {2009},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.80.104009},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.80.104009}
}
@article{Yagi:2013du,
      author         = "Yagi, Kent",
      title          = "{Scientific Potential of DECIGO Pathfinder and Testing GR
                        with Space-Borne Gravitational Wave Interferometers}",
      journal        = "Int. J. Mod. Phys.",
      volume         = "D22",
      year           = "2013",
      pages          = "1341013",
      doi            = "10.1142/S0218271813410137",
      eprint         = "1302.2388",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = ARXIV:1302.2388;%%"
}
@article{Sathyaprakash:2012jk,
      author         = "Sathyaprakash, B. and others",
      title          = "{Scientific Objectives of Einstein Telescope}",
      booktitle      = "{Gravitational waves. Numerical relativity - data
                        analysis. Proceedings, 9th Edoardo Amaldi Conference,
                        Amaldi 9, and meeting, NRDA 2011, Cardiff, UK, July 10-15,
                        2011}",
      journal        = "Class. Quant. Grav.",
      volume         = "29",
      year           = "2012",
      pages          = "124013",
      doi            = "10.1088/0264-9381/29/12/124013,
                        10.1088/0264-9381/30/7/079501",
      note           = "[Erratum: Class. Quant. Grav.30,079501(2013)]",
      eprint         = "1206.0331",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = ARXIV:1206.0331;%%"
}





@article{Linde:1981zj,
      author         = "Linde, Andrei D.",
      title          = "{Decay of the False Vacuum at Finite Temperature}",
      journal        = "Nucl. Phys.",
      volume         = "B216",
      year           = "1983",
      pages          = "421",
      doi            = "10.1016/0550-3213(83)90293-6,
                        10.1016/0550-3213(83)90072-X",
      note           = "[Erratum: Nucl. Phys.B223,544(1983)]",
      reportNumber   = "LEBEDEV-81-265",
      SLACcitation   = "%%CITATION = NUPHA,B216,421;%%"
}




@article{Linde:1980tt,
      author         = "Linde, Andrei D.",
      title          = "{Fate of the False Vacuum at Finite Temperature: Theory
                        and Applications}",
      journal        = "Phys. Lett.",
      volume         = "100B",
      year           = "1981",
      pages          = "37-40",
      doi            = "10.1016/0370-2693(81)90281-1",
      reportNumber   = "LEBEDEV-80-92",
      SLACcitation   = "%%CITATION = PHLTA,100B,37;%%"
}


@article{Kosowsky:1991ua,
      author         = "Kosowsky, Arthur and Turner, Michael S. and Watkins,
                        Richard",
      title          = "{Gravitational radiation from colliding vacuum bubbles}",
      journal        = "Phys. Rev.",
      volume         = "D45",
      year           = "1992",
      pages          = "4514-4535",
      doi            = "10.1103/PhysRevD.45.4514",
      reportNumber   = "FERMILAB-PUB-91-323-A",
      SLACcitation   = "%%CITATION = PHRVA,D45,4514;%%"
}


@article{Kosowsky:1992rz,
      author         = "Kosowsky, Arthur and Turner, Michael S. and Watkins,
                        Richard",
      title          = "{Gravitational waves from first order cosmological phase
                        transitions}",
      journal        = "Phys. Rev. Lett.",
      volume         = "69",
      year           = "1992",
      pages          = "2026-2029",
      doi            = "10.1103/PhysRevLett.69.2026",
      reportNumber   = "FERMILAB-PUB-91-333-A-REV, FERMILAB-PUB-91-333-A",
      SLACcitation   = "%%CITATION = PRLTA,69,2026;%%"
}


@article{Kosowsky:1992vn,
      author         = "Kosowsky, Arthur and Turner, Michael S.",
      title          = "{Gravitational radiation from colliding vacuum bubbles:
                        envelope approximation to many bubble collisions}",
      journal        = "Phys. Rev.",
      volume         = "D47",
      year           = "1993",
      pages          = "4372-4391",
      doi            = "10.1103/PhysRevD.47.4372",
      eprint         = "astro-ph/9211004",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "FERMILAB-PUB-92-295-A",
      SLACcitation   = "%%CITATION = ASTRO-PH/9211004;%%"
}


@article{Kamionkowski:1993fg,
      author         = "Kamionkowski, Marc and Kosowsky, Arthur and Turner,
                        Michael S.",
      title          = "{Gravitational radiation from first order phase
                        transitions}",
      journal        = "Phys. Rev.",
      volume         = "D49",
      year           = "1994",
      pages          = "2837-2851",
      doi            = "10.1103/PhysRevD.49.2837",
      eprint         = "astro-ph/9310044",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "IASSNS-HEP-93-44, FERMILAB-PUB-93-235-A",
      SLACcitation   = "%%CITATION = ASTRO-PH/9310044;%%"
}


@article{Kosowsky:2001xp,
      author         = "Kosowsky, Arthur and Mack, Andrew and Kahniashvili,
                        Tinatin",
      title          = "{Gravitational radiation from cosmological turbulence}",
      journal        = "Phys. Rev.",
      volume         = "D66",
      year           = "2002",
      pages          = "024030",
      doi            = "10.1103/PhysRevD.66.024030",
      eprint         = "astro-ph/0111483",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "RAP-334",
      SLACcitation   = "%%CITATION = ASTRO-PH/0111483;%%"
}


@article{Konstandin:2017sat,
      author         = "Konstandin, Thomas",
      title          = "{Gravitational radiation from a bulk flow model}",
      journal        = "JCAP",
      volume         = "1803",
      year           = "2018",
      number         = "03",
      pages          = "047",
      doi            = "10.1088/1475-7516/2018/03/047",
      eprint         = "1712.06869",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "DESY-17-227",
      SLACcitation   = "%%CITATION = ARXIV:1712.06869;%%"
}


@article{Jinno:2017fby,
      author         = "Jinno, Ryusuke and Takimoto, Masahiro",
      title          = "{Gravitational waves from bubble dynamics: Beyond the
                        Envelope}",
      journal        = "JCAP",
      volume         = "1901",
      year           = "2019",
      pages          = "060",
      doi            = "10.1088/1475-7516/2019/01/060",
      eprint         = "1707.03111",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CTPU-17-26, KEK-TH-1986",
      SLACcitation   = "%%CITATION = ARXIV:1707.03111;%%"
}


@article{Enqvist:1991xw,
      author         = "Enqvist, K. and Ignatius, J. and Kajantie, K. and
                        Rummukainen, K.",
      title          = "{Nucleation and bubble growth in a first order
                        cosmological electroweak phase transition}",
      journal        = "Phys. Rev.",
      volume         = "D45",
      year           = "1992",
      pages          = "3415-3428",
      doi            = "10.1103/PhysRevD.45.3415",
      reportNumber   = "HU-TFT-91-35",
      SLACcitation   = "%%CITATION = PHRVA,D45,3415;%%"
}


@article{Caprini:2009yp,
      author         = "Caprini, Chiara and Durrer, Ruth and Servant, Geraldine",
      title          = "{The stochastic gravitational wave background from
                        turbulence and magnetic fields generated by a first-order
                        phase transition}",
      journal        = "JCAP",
      volume         = "0912",
      year           = "2009",
      pages          = "024",
      doi            = "10.1088/1475-7516/2009/12/024",
      eprint         = "0909.0622",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:0909.0622;%%"
}


@article{Konstandin:2014zta,
      author         = "Konstandin, Thomas and Nardini, Germano and Rues, Ingo",
      title          = "{From Boltzmann equations to steady wall velocities}",
      journal        = "JCAP",
      volume         = "1409",
      year           = "2014",
      number         = "09",
      pages          = "028",
      doi            = "10.1088/1475-7516/2014/09/028",
      eprint         = "1407.3132",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-14-127, NSF-KITP-14-089",
      SLACcitation   = "%%CITATION = ARXIV:1407.3132;%%"
}



@article{Leitao:2014pda,
      author         = "Leitao, Leonardo and Megevand, Ariel",
      title          = "{Hydrodynamics of phase transition fronts and the speed
                        of sound in the plasma}",
      journal        = "Nucl. Phys.",
      volume         = "B891",
      year           = "2015",
      pages          = "159-199",
      doi            = "10.1016/j.nuclphysb.2014.12.008",
      eprint         = "1410.3875",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1410.3875;%%"
}


@article{Bernard:2004je,
      author         = "Bernard, C. and Burch, T. and Gregory, E. B. and
                        Toussaint, D. and DeTar, Carleton E. and Osborn, J. and
                        Gottlieb, Steven and Heller, U. M. and Sugar, R.",
      title          = "{QCD thermodynamics with three flavors of improved
                        staggered quarks}",
      collaboration  = "MILC",
      journal        = "Phys. Rev.",
      volume         = "D71",
      year           = "2005",
      pages          = "034504",
      doi            = "10.1103/PhysRevD.71.034504",
      eprint         = "hep-lat/0405029",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      SLACcitation   = "%%CITATION = HEP-LAT/0405029;%%"
}



@article{Rummukainen:1998as,
      author         = "Rummukainen, K. and Tsypin, M. and Kajantie, K. and
                        Laine, M. and Shaposhnikov, Mikhail E.",
      title          = "{The Universality class of the electroweak theory}",
      journal        = "Nucl. Phys.",
      volume         = "B532",
      year           = "1998",
      pages          = "283-314",
      doi            = "10.1016/S0550-3213(98)00494-5",
      eprint         = "hep-lat/9805013",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      reportNumber   = "CERN-TH-98-08, NORDITA-98-30-HE",
      SLACcitation   = "%%CITATION = HEP-LAT/9805013;%%"
}

@article{Csikor:1998eu,
      author         = "Csikor, F. and Fodor, Z. and Heitger, J.",
      title          = "{Endpoint of the hot electroweak phase transition}",
      journal        = "Phys. Rev. Lett.",
      volume         = "82",
      year           = "1999",
      pages          = "21-24",
      doi            = "10.1103/PhysRevLett.82.21",
      eprint         = "hep-ph/9809291",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ITP-BUDAPEST-541, KEK-TH-580, KEK-PREPRINT-98-160,
                        MS-TPI-98-16",
      SLACcitation   = "%%CITATION = HEP-PH/9809291;%%"
}




@article{Aoki:2006we,
      author         = "Aoki, Y. and Endrodi, G. and Fodor, Z. and Katz, S. D.
                        and Szabo, K. K.",
      title          = "{The Order of the quantum chromodynamics transition
                        predicted by the standard model of particle physics}",
      journal        = "Nature",
      volume         = "443",
      year           = "2006",
      pages          = "675-678",
      doi            = "10.1038/nature05120",
      eprint         = "hep-lat/0611014",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      SLACcitation   = "%%CITATION = HEP-LAT/0611014;%%"
}

@article{Cheng:2006qk,
      author         = "Cheng, M. and others",
      title          = "{The Transition temperature in QCD}",
      journal        = "Phys. Rev.",
      volume         = "D74",
      year           = "2006",
      pages          = "054507",
      doi            = "10.1103/PhysRevD.74.054507",
      eprint         = "hep-lat/0608013",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      reportNumber   = "BNL-NT-06-27, BI-TP-2006-31, CU-TP-1158",
      SLACcitation   = "%%CITATION = HEP-LAT/0608013;%%"
}

%%% contains utf-8, see: http://inspirehep.net/info/faq/general#utf8
%%% add \usepackage[utf8]{inputenc} to your latex preamble

@article{Croon:2018erz,
      author         = "Croon, Djuna and Sanz, Ver�nica and White, Graham",
      title          = "{Model Discrimination in Gravitational Wave spectra from
                        Dark Phase Transitions}",
      journal        = "JHEP",
      volume         = "08",
      year           = "2018",
      pages          = "203",
      doi            = "10.1007/JHEP08(2018)203",
      eprint         = "1806.02332",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1806.02332;%%"
}


@article{Moore:2014lga,
      author         = "Moore, C. J. and Cole, R. H. and Berry, C. P. L.",
      title          = "{Gravitational-wave sensitivity curves}",
      journal        = "Class. Quant. Grav.",
      volume         = "32",
      year           = "2015",
      number         = "1",
      pages          = "015014",
      doi            = "10.1088/0264-9381/32/1/015014",
      eprint         = "1408.0740",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      reportNumber   = "LIGO-P1400129",
      SLACcitation   = "%%CITATION = ARXIV:1408.0740;%%"
}



@article{Guth:1981uk,
      author         = "Guth, Alan H. and Weinberg, Erick J.",
      title          = "{Cosmological Consequences of a First Order Phase
                        Transition in the SU(5) Grand Unified Model}",
      journal        = "Phys. Rev.",
      volume         = "D23",
      year           = "1981",
      pages          = "876",
      doi            = "10.1103/PhysRevD.23.876",
      reportNumber   = "CU-TP-183",
      SLACcitation   = "%%CITATION = PHRVA,D23,876;%%"
}


@article{Guth:1979bh,
      author         = "Guth, Alan H. and Tye, S. H. H.",
      title          = "{Phase Transitions and Magnetic Monopole Production in
                        the Very Early Universe}",
      journal        = "Phys. Rev. Lett.",
      volume         = "44",
      year           = "1980",
      pages          = "631",
      doi            = "10.1103/PhysRevLett.44.631, 10.1103/PhysRevLett.44.963.2",
      note           = "[Erratum: Phys. Rev. Lett.44,963(1980)]",
      reportNumber   = "SLAC-PUB-2448, CLNS-79-441",
      SLACcitation   = "%%CITATION = PRLTA,44,631;%%"
}

@article{Caprini:2009fx,
      author         = "Caprini, Chiara and Durrer, Ruth and Konstandin, Thomas
                        and Servant, Geraldine",
      title          = "{General Properties of the Gravitational Wave Spectrum
                        from Phase Transitions}",
      journal        = "Phys. Rev.",
      volume         = "D79",
      year           = "2009",
      pages          = "083519",
      doi            = "10.1103/PhysRevD.79.083519",
      eprint         = "0901.1661",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:0901.1661;%%"
}
@article{Ellis:2019tjf,
      author         = "Ellis, John and Fairbairn, Malcolm and Lewicki, Marek and
                        Vaskonen, Ville and Wickens, Alastair",
      title          = "{Intergalactic Magnetic Fields from First-Order Phase
                        Transitions}",
      journal        = "JCAP",
      volume         = "1909",
      year           = "2019",
      number         = "09",
      pages          = "019",
      doi            = "10.1088/1475-7516/2019/09/019",
      eprint         = "1907.04315",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1907.04315;%%"
}
@article{Jedamzik:1999am,
      author         = "Jedamzik, K. and Niemeyer, Jens C.",
      title          = "{Primordial black hole formation during first order phase
                        transitions}",
      journal        = "Phys. Rev.",
      volume         = "D59",
      year           = "1999",
      pages          = "124014",
      doi            = "10.1103/PhysRevD.59.124014",
      eprint         = "astro-ph/9901293",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/9901293;%%"
}
@article{Konstandin:2011dr,
      author         = "Konstandin, Thomas and Servant, Geraldine",
      title          = "{Cosmological Consequences of Nearly Conformal Dynamics
                        at the TeV scale}",
      journal        = "JCAP",
      volume         = "1112",
      year           = "2011",
      pages          = "009",
      doi            = "10.1088/1475-7516/2011/12/009",
      eprint         = "1104.4791",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1104.4791;%%"
}
@article{Konstandin:2011ds,
      author         = "Konstandin, Thomas and Servant, Geraldine",
      title          = "{Natural Cold Baryogenesis from Strongly Interacting
                        Electroweak Symmetry Breaking}",
      journal        = "JCAP",
      volume         = "1107",
      year           = "2011",
      pages          = "024",
      doi            = "10.1088/1475-7516/2011/07/024",
      eprint         = "1104.4793",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1104.4793;%%"
}
@article{Gildener:1976ih,
      author         = "Gildener, Eldad and Weinberg, Steven",
      title          = "{Symmetry Breaking and Scalar Bosons}",
      journal        = "Phys. Rev.",
      volume         = "D13",
      year           = "1976",
      pages          = "3333",
      doi            = "10.1103/PhysRevD.13.3333",
      reportNumber   = "PRINT-76-0068 (HARVARD)",
      SLACcitation   = "%%CITATION = PHRVA,D13,3333;%%"
}
@article{GINSPARG1980388,
title = "First and second order phase transitions in gauge theories at finite temperature",
journal = "Nuclear Physics B",
volume = "170",
number = "3",
pages = "388 - 408",
year = "1980",
issn = "0550-3213",
doi = "https://doi.org/10.1016/0550-3213(80)90418-6",
url = "http://www.sciencedirect.com/science/article/pii/0550321380904186",
author = "Paul Ginsparg",
abstract = "We consider in general the nature of the phase transition which occurs in 4D gauge theories coupled to scalar and spinor fields at finite temperature. It is shown that the critical behavior can be isolated in an effective 3D theory of the zero frequency mode whose lagrangian may be calculated explicitly in weak coupling perturbation theory. This lagrangian, in turn, may be investigated by means of standard ϵ-expansion techniques. Theories with an asymptotically free gauge coupling constant possess no stable fixed point in the ϵ-expansion and are inferred to have weakly first-order phase transitions; theories not satisfying this condition may have second-order transitions."
}
@article{Arnold:1992rz,
      author         = "Arnold, Peter Brockway and Espinosa, Olivier",
      title          = "{The Effective potential and first order phase
                        transitions: Beyond leading-order}",
      journal        = "Phys. Rev.",
      volume         = "D47",
      year           = "1993",
      pages          = "3546",
      doi            = "10.1103/physrevd.50.6662.2, 10.1103/PhysRevD.47.3546",
      note           = "[Erratum: Phys. Rev.D50,6662(1994)]",
      eprint         = "hep-ph/9212235",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UW-PT-92-18, USM-TH-60",
      SLACcitation   = "%%CITATION = HEP-PH/9212235;%%"
}
@article{Weinberg:1974hy,
      author         = "Weinberg, Steven",
      title          = "{Gauge and Global Symmetries at High Temperature}",
      journal        = "Phys. Rev.",
      volume         = "D9",
      year           = "1974",
      pages          = "3357-3378",
      doi            = "10.1103/PhysRevD.9.3357",
      reportNumber   = "PRINT-74-0689 (HARVARD)",
      SLACcitation   = "%%CITATION = PHRVA,D9,3357;%%"
}
@inproceedings{Gleiser:1994ue,
      author         = "Gleiser, Marcelo",
      title          = "{On the strength of first order phase transitions}",
      booktitle      = "{1st International Conference on Strong and Electroweak
                        Matter (SEWM 1994) Sintra, Portugal, March 23-25, 1994}",
      year           = "1994",
      pages          = "63-78",
      eprint         = "hep-ph/9405269",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DART-HEP-94-02",
      SLACcitation   = "%%CITATION = HEP-PH/9405269;%%"
}
@article{Miura:2018dsy,
      author         = "Miura, Kohtaroh and Ohki, Hiroshi and Otani, Saeko and
                        Yamawaki, Koichi",
      title          = "{Gravitational Waves from Walking Technicolor}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2019",
      pages          = "194",
      doi            = "10.1007/JHEP10(2019)194",
      eprint         = "1811.05670",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MITP/18-112",
      SLACcitation   = "%%CITATION = ARXIV:1811.05670;%%"
}
@article{Appelquist:1996dq,
      author         = "Appelquist, Thomas and Terning, John and Wijewardhana, L.
                        C. R.",
      title          = "{The Zero temperature chiral phase transition in SU(N)
                        gauge theories}",
      journal        = "Phys. Rev. Lett.",
      volume         = "77",
      year           = "1996",
      pages          = "1214-1217",
      doi            = "10.1103/PhysRevLett.77.1214",
      eprint         = "hep-ph/9602385",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "YCTP-P2-96, BUHEP-96-3, UCTP-002-96",
      SLACcitation   = "%%CITATION = HEP-PH/9602385;%%"
}
@article{Aoki:2013xza,
      author         = "Aoki, Yasumichi and Aoyama, Tatsumi and Kurachi, Masafumi
                        and Maskawa, Toshihide and Nagai, Kei-ichi and Ohki,
                        Hiroshi and Shibata, Akihiro and Yamawaki, Koichi and
                        Yamazaki, Takeshi",
      title          = "{Walking signals in $N_f=8$ QCD on the lattice}",
      collaboration  = "LatKMI",
      journal        = "Phys. Rev.",
      volume         = "D87",
      year           = "2013",
      number         = "9",
      pages          = "094511",
      doi            = "10.1103/PhysRevD.87.094511",
      eprint         = "1302.6859",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      reportNumber   = "KEK-PREPRINT-2012-47",
      SLACcitation   = "%%CITATION = ARXIV:1302.6859;%%"
}
@article{Appelquist:2014zsa,
      author         = "Appelquist, T. and others",
      title          = "{Lattice simulations with eight flavors of domain wall
                        fermions in SU(3) gauge theory}",
      collaboration  = "LSD",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "11",
      pages          = "114502",
      doi            = "10.1103/PhysRevD.90.114502",
      eprint         = "1405.4752",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      reportNumber   = "LLNL-JRNL-665913",
      SLACcitation   = "%%CITATION = ARXIV:1405.4752;%%"
}
@article{Hasenfratz:2014rna,
      author         = "Hasenfratz, Anna and Schaich, David and Veernala, Aarti",
      title          = "{Nonperturbative $\beta$ function of eight-flavor SU(3)
                        gauge theory}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2015",
      pages          = "143",
      doi            = "10.1007/JHEP06(2015)143",
      eprint         = "1410.5886",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      SLACcitation   = "%%CITATION = ARXIV:1410.5886;%%"
}
@article{Appelquist:2016viq,
      author         = "Appelquist, Thomas and others",
      title          = "{Strongly interacting dynamics and the search for new
                        physics at the LHC}",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "11",
      pages          = "114514",
      doi            = "10.1103/PhysRevD.93.114514",
      eprint         = "1601.04027",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      reportNumber   = "EDINBURGH-2016-01, LLNL-JRNL-680732, NSF-KITP-16-004",
      SLACcitation   = "%%CITATION = ARXIV:1601.04027;%%"
}
@article{Appelquist:2018yqe,
      author         = "Appelquist, T. and others",
      title          = "{Nonperturbative investigations of SU(3) gauge theory
                        with eight dynamical flavors}",
      collaboration  = "Lattice Strong Dynamics",
      journal        = "Phys. Rev.",
      volume         = "D99",
      year           = "2019",
      number         = "1",
      pages          = "014509",
      doi            = "10.1103/PhysRevD.99.014509",
      eprint         = "1807.08411",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      reportNumber   = "RBRC-1286; LLNL-JRNL-753511",
      SLACcitation   = "%%CITATION = ARXIV:1807.08411;%%"
}
%%% contains utf-8, see: https://inspirehep.net/info/faq/general#utf8
%%% add \usepackage[utf8]{inputenc} to your latex preamble

@article{Prokopec:2018tnq,
      author         = "Prokopec, Tomislav and Rezacek, Jonas and Świeżewska,
                        Bogumiła",
      title          = "{Gravitational waves from conformal symmetry breaking}",
      journal        = "JCAP",
      volume         = "1902",
      year           = "2019",
      number         = "02",
      pages          = "009",
      doi            = "10.1088/1475-7516/2019/02/009",
      eprint         = "1809.11129",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1809.11129;%%"
}
%%% contains utf-8, see: https://inspirehep.net/info/faq/general#utf8
%%% add \usepackage[utf8]{inputenc} to your latex preamble


@article{Thrane:2013oya,
      author         = "Thrane, Eric and Romano, Joseph D.",
      title          = "{Sensitivity curves for searches for gravitational-wave
                        backgrounds}",
      journal        = "Phys. Rev.",
      volume         = "D88",
      year           = "2013",
      number         = "12",
      pages          = "124032",
      doi            = "10.1103/PhysRevD.88.124032",
      eprint         = "1310.5300",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1310.5300;%%"
}

@article{Marfatia:2020bcs,
    author = "Marfatia, Danny and Tseng, Po-Yan",
    title = "{Gravitational wave signals of dark matter freeze-out}",
    eprint = "2006.07313",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}

@article{Long:2017rdo,
    author = "Long, Andrew J. and Tesi, Andrea and Wang, Lian-Tao",
    title = "{Baryogenesis at a Lepton-Number-Breaking Phase Transition}",
    eprint = "1703.04902",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP10(2017)095",
    journal = "JHEP",
    volume = "10",
    pages = "095",
    year = "2017"
}


@article{PhysRevLett.125.151102,
  title = {Filtered Dark Matter at a First Order Phase Transition},
  author = {Baker, Michael J. and Kopp, Joachim and Long, Andrew J.},
  journal = {Phys. Rev. Lett.},
  volume = {125},
  issue = {15},
  pages = {151102},
  numpages = {7},
  year = {2020},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.125.151102},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.125.151102}
}
@article{PhysRevD.101.043527,
  title = {Spontaneous freeze out of dark matter from an early thermal phase transition},
  author = {Heurtier, Lucien and Partouche, Herv\'e},
  journal = {Phys. Rev. D},
  volume = {101},
  issue = {4},
  pages = {043527},
  numpages = {15},
  year = {2020},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.101.043527},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.101.043527}
}
@article{PhysRevLett.64.615,
  title = {Unitarity limits on the mass and radius of dark-matter particles},
  author = {Griest, Kim and Kamionkowski, Marc},
  journal = {Phys. Rev. Lett.},
  volume = {64},
  issue = {6},
  pages = {615--618},
  numpages = {0},
  year = {1990},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.64.615},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.64.615}
}
@article{Darme:2019wpd,
    author = "Darm\'e, Luc and Hryczuk, Andrzej and Karamitros, Dimitrios and Roszkowski, Leszek",
    title = "{Forbidden frozen-in dark matter}",
    eprint = "1908.05685",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP11(2019)159",
    journal = "JHEP",
    volume = "11",
    pages = "159",
    year = "2019"
}
@article{Baker:2016xzo,
    author = "Baker, Michael J. and Kopp, Joachim",
    title = "{Dark Matter Decay between Phase Transitions at the Weak Scale}",
    eprint = "1608.07578",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MITP-16-090",
    doi = "10.1103/PhysRevLett.119.061801",
    journal = "Phys. Rev. Lett.",
    volume = "119",
    number = "6",
    pages = "061801",
    year = "2017"
}
@article{Baker:2018vos,
    author = "Baker, Michael J. and Mittnacht, Lukas",
    title = "{Variations on the Vev Flip-Flop: Instantaneous Freeze-out and Decaying Dark Matter}",
    eprint = "1811.03101",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MITP/18-109, ZU-TH-41-18",
    doi = "10.1007/JHEP05(2019)070",
    journal = "JHEP",
    volume = "05",
    pages = "070",
    year = "2019"
}
@article{Laurent:2020gpg,
    author = "Laurent, Benoit and Cline, James M.",
    title = "{Fluid equations for fast-moving electroweak bubble walls}",
    eprint = "2007.10935",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.102.063516",
    journal = "Phys. Rev. D",
    volume = "102",
    number = "6",
    pages = "063516",
    year = "2020"
}


@article{Azatov:2021irb,
    author = "Azatov, Aleksandr and Vanvlasselaer, Miguel and Yin, Wen",
    title = "{Baryogenesis via relativistic bubble walls}",
    eprint = "2106.14913",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SISSA 13/2021/FISI TU-1127",
    doi = "10.1007/JHEP10(2021)043",
    journal = "JHEP",
    volume = "10",
    pages = "043",
    year = "2021"
}
@article{Azatov:2022tii,
    author = "Azatov, Aleksandr and Barni, Giulio and Chakraborty, Sabyasachi and Vanvlasselaer, Miguel and Yin, Wen",
    title = "{Ultra-relativistic bubbles from the simplest Higgs portal and their cosmological consequences}",
    eprint = "2207.02230",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SISSA 12/2022/FISI TU-1157",
    doi = "10.1007/JHEP10(2022)017",
    journal = "JHEP",
    volume = "10",
    pages = "017",
    year = "2022"
}
@article{Caprini:2019egz,
    author = "Caprini, Chiara and others",
    title = "{Detecting gravitational waves from cosmological phase transitions with LISA: an update}",
    eprint = "1910.13125",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "DESY-19-159, IPPP/19/27, HIP-2019-14/TH, MITP/19-066, IFT-UAM/CSIC-19-139",
    doi = "10.1088/1475-7516/2020/03/024",
    journal = "JCAP",
    volume = "03",
    pages = "024",
    year = "2020"
}

@article{Vanvlasselaer:2020niz,
    author = "Azatov, Aleksandr and Vanvlasselaer, Miguel",
    title = "{Bubble wall velocity: heavy physics effects}",
    eprint = "2010.02590",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SISSA 247/2020/FISI",
    doi = "10.1088/1475-7516/2021/01/058",
    journal = "JCAP",
    volume = "01",
    pages = "058",
    year = "2021"
}


@article{Srednicki:1988ce,
    author = "Srednicki, Mark and Watkins, Richard and Olive, Keith A.",
    editor = "Srednicki, M.A.",
    title = "{Calculations of Relic Densities in the Early Universe}",
    reportNumber = "UMN-TH-646/88",
    doi = "10.1016/0550-3213(88)90099-5",
    journal = "Nucl. Phys. B",
    volume = "310",
    pages = "693",
    year = "1988"
}

@article{GONDOLO1991145,
title = "Cosmic abundances of stable particles: Improved analysis",
journal = "Nuclear Physics B",
volume = "360",
number = "1",
pages = "145 - 179",
year = "1991",
issn = "0550-3213",
doi = "https://doi.org/10.1016/0550-3213(91)90438-4",
url = "http://www.sciencedirect.com/science/article/pii/0550321391904384",
author = "Paolo Gondolo and Graciela Gelmini",
abstract = "An exact relativistic single-integral formula for the thermal average of the annihilation cross section times velocity, the key quantity in the determination of the cosmic relic abundance of a species, is obtained. Since it does not require expansion of the cross section at low relative velocity, it can also be used when the cross section varies rapidly with energy, e.g. near the formation of a resonance or the opening of a new annihilation channel. We discuss approximate formulas in these cases, and we find that dips in the relic density near resonances are significantly broader and shallower than previously thought and that spurious reductions near thresholds disappear."
}
@article{Griest:1990kh,
    author = "Griest, Kim and Seckel, David",
    title = "{Three exceptions in the calculation of relic abundances}",
    reportNumber = "CFPA-TH-90-001A, BA-90-79",
    doi = "10.1103/PhysRevD.43.3191",
    journal = "Phys. Rev. D",
    volume = "43",
    pages = "3191--3203",
    year = "1991"
}


@article{Chung:1998zb,
    author = "Chung, Daniel J.H. and Kolb, Edward W. and Riotto, Antonio",
    title = "{Superheavy dark matter}",
    eprint = "hep-ph/9802238",
    archivePrefix = "arXiv",
    reportNumber = "FERMILAB-PUB-98-021-A, CERN-TH-98-37, OUTP-98-02-P, FERMILAB-FERMILAB-PUB-98-021-A, CERN-CERN-TH-98-37, OXFORD-U. --OUTP-98-02-P",
    doi = "10.1103/PhysRevD.59.023501",
    journal = "Phys. Rev. D",
    volume = "59",
    pages = "023501",
    year = "1998"
}

@article{Allahverdi:2018iod,
    author = "Allahverdi, Rouzbeh and Dutta, Koushik and Maharana, Anshuman",
    title = "{Constraining Non-thermal Dark Matter by CMB}",
    eprint = "1808.02659",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2018/10/038",
    journal = "JCAP",
    volume = "10",
    pages = "038",
    year = "2018"
}
@article{Hall:2009bx,
    author = "Hall, Lawrence J. and Jedamzik, Karsten and March-Russell, John and West, Stephen M.",
    title = "{Freeze-In Production of FIMP Dark Matter}",
    eprint = "0911.1120",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "OUTP-09-18-P, UCB-PTH-09-32",
    doi = "10.1007/JHEP03(2010)080",
    journal = "JHEP",
    volume = "03",
    pages = "080",
    year = "2010"
}

@article{Chu:2013jja,
    author = "Chu, Xiaoyong and Mambrini, Yann and Quevillon, J\'er\'emie and Zaldivar, Bryan",
    title = "{Thermal and non-thermal production of dark matter via Z'-portal(s)}",
    eprint = "1306.4677",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2014/01/034",
    journal = "JCAP",
    volume = "01",
    pages = "034",
    year = "2014"
}

@article{Chway:2019kft,
    author = "Chway, Dongjin and Jung, Tae Hyun and Shin, Chang Sub",
    title = "{Dark matter filtering-out effect during a first-order phase transition}",
    eprint = "1912.04238",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CTPU-19-37",
    doi = "10.1103/PhysRevD.101.095019",
    journal = "Phys. Rev. D",
    volume = "101",
    number = "9",
    pages = "095019",
    year = "2020"
}
@article{Hui:1998dc,
    author = "Hui, Lam and Stewart, Ewan D.",
    title = "{Superheavy dark matter from thermal inflation}",
    eprint = "hep-ph/9812345",
    archivePrefix = "arXiv",
    reportNumber = "FERMILAB-PUB-98-397-A",
    doi = "10.1103/PhysRevD.60.023518",
    journal = "Phys. Rev. D",
    volume = "60",
    pages = "023518",
    year = "1999"
}
@article{Hambye:2018qjv,
    author = "Hambye, Thomas and Strumia, Alessandro and Teresi, Daniele",
    title = "{Super-cool Dark Matter}",
    eprint = "1805.01473",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "ULB-TH/18-06, CERN-TH-2018-110, IFUP-TH/2018, ULB-TH-18-06",
    doi = "10.1007/JHEP08(2018)188",
    journal = "JHEP",
    volume = "08",
    pages = "188",
    year = "2018"
}
@article{Cline:2020jre,
    author = "Cline, James M. and Kainulainen, Kimmo",
    title = "{Electroweak baryogenesis at high bubble wall velocities}",
    eprint = "2001.00568",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2019-227",
    doi = "10.1103/PhysRevD.101.063525",
    journal = "Phys. Rev. D",
    volume = "101",
    number = "6",
    pages = "063525",
    year = "2020"
}




@article{Cline:2017jvp,
    author = "Cline, James M.",
    editor = "Auge, Etienne and Dumarchez, Jacques and Tran Thanh Van, Jean",
    title = "{Is electroweak baryogenesis dead?}",
    eprint = "1704.08911",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2017-096",
    doi = "10.1098/rsta.2017.0116",
    journal = "Phil. Trans. Roy. Soc. Lond. A",
    volume = "376",
    number = "2114",
    pages = "20170116",
    year = "2018"
}
@article{Caprini:2011uz,
    author = "Caprini, Chiara and No, Jose M.",
    title = "{Supersonic Electroweak Baryogenesis: Achieving Baryogenesis for Fast Bubble Walls}",
    eprint = "1111.1726",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SACLAY-T11-209, ULB-TH-11-25",
    doi = "10.1088/1475-7516/2012/01/031",
    journal = "JCAP",
    volume = "01",
    pages = "031",
    year = "2012"
}

@article{Murayama:2002je,
    author = "Murayama, Hitoshi and Pierce, Aaron",
    title = "{Realistic Dirac leptogenesis}",
    eprint = "hep-ph/0206177",
    archivePrefix = "arXiv",
    reportNumber = "UCB-PTH-02-26, LBNL-50854",
    doi = "10.1103/PhysRevLett.89.271601",
    journal = "Phys. Rev. Lett.",
    volume = "89",
    pages = "271601",
    year = "2002"
}
@article{Dick:1999je,
    author = "Dick, Karin and Lindner, Manfred and Ratz, Michael and Wright, David",
    title = "{Leptogenesis with Dirac neutrinos}",
    eprint = "hep-ph/9907562",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevLett.84.4039",
    journal = "Phys. Rev. Lett.",
    volume = "84",
    pages = "4039--4042",
    year = "2000"
}





@article{Petraki:2013wwa,
    author = "Petraki, Kalliopi and Volkas, Raymond R.",
    title = "{Review of asymmetric dark matter}",
    eprint = "1305.4939",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "NIKHEF-2013-016",
    doi = "10.1142/S0217751X13300287",
    journal = "Int. J. Mod. Phys. A",
    volume = "28",
    pages = "1330028",
    year = "2013"
}

@article{Katz:2016adq,
    author = "Katz, Andrey and Riotto, Antonio",
    title = "{Baryogenesis and Gravitational Waves from Runaway Bubble Collisions}",
    eprint = "1608.00583",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2016-173",
    doi = "10.1088/1475-7516/2016/11/011",
    journal = "JCAP",
    volume = "11",
    pages = "011",
    year = "2016"
}

@article{Azatov:2020nbe,
    author = "Azatov, Aleksandr and Vanvlasselaer, Miguel",
    title = "{Phase transitions in perturbative walking dynamics}",
    eprint = "2003.10265",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SISSA 03/2020/FISI",
    doi = "10.1007/JHEP09(2020)085",
    journal = "JHEP",
    volume = "09",
    pages = "085",
    year = "2020"
}

@article{Falkowski:2012fb,
    author = "Falkowski, Adam and No, Jose M.",
    title = "{Non-thermal Dark Matter Production from the Electroweak Phase Transition: Multi-TeV WIMPs and 'Baby-Zillas'}",
    eprint = "1211.5615",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "ULB-TH-12-18, LPT-12-113",
    doi = "10.1007/JHEP02(2013)034",
    journal = "JHEP",
    volume = "02",
    pages = "034",
    year = "2013"
}

@article{Espinosa:2007qk,
    author = "Espinosa, Jose Ramon and Quiros, Mariano",
    title = "{Novel Effects in Electroweak Breaking from a Hidden Sector}",
    eprint = "hep-ph/0701145",
    archivePrefix = "arXiv",
    reportNumber = "IFT-UAM-CSIC-07-01, UAB-FT-623",
    doi = "10.1103/PhysRevD.76.076004",
    journal = "Phys. Rev. D",
    volume = "76",
    pages = "076004",
    year = "2007"
}

@article{Watkins:1991zt,
    author = "Watkins, Richard and Widrow, Lawrence M.",
    title = "{Aspects of reheating in first order inflation}",
    reportNumber = "FERMILAB-PUB-91-164-A",
    doi = "10.1016/0550-3213(92)90362-F",
    journal = "Nucl. Phys. B",
    volume = "374",
    pages = "446--468",
    year = "1992"
}

@article{Cai:2020djd,
    author = "Cai, Rong-Gen and Wang, Shao-Jiang",
    title = "{Effective picture of bubble expansion}",
    eprint = "2011.11451",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    month = "11",
    year = "2020"
}

@article{Arcadi:2016qoz,
    author = "Arcadi, Giorgio and Gross, Christian and Lebedev, Oleg and Pokorski, Stefan and Toma, Takashi",
    title = "{Evading Direct Dark Matter Detection in Higgs Portal Models}",
    eprint = "1611.09675",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "TUM-HEP-1072-16, HIP-2016-38-TH",
    doi = "10.1016/j.physletb.2017.03.044",
    journal = "Phys. Lett. B",
    volume = "769",
    pages = "129--133",
    year = "2017"
}
@article{Pospelov:2007mp,
    author = "Pospelov, Maxim and Ritz, Adam and Voloshin, Mikhail B.",
    title = "{Secluded WIMP Dark Matter}",
    eprint = "0711.4866",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1016/j.physletb.2008.02.052",
    journal = "Phys. Lett. B",
    volume = "662",
    pages = "53--61",
    year = "2008"
}

@article{Baer:2014eja,
    author = "Baer, Howard and Choi, Ki-Young and Kim, Jihn E. and Roszkowski, Leszek",
    title = "{Dark matter production in the early Universe: beyond the thermal WIMP paradigm}",
    eprint = "1407.0017",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1016/j.physrep.2014.10.002",
    journal = "Phys. Rept.",
    volume = "555",
    pages = "1--60",
    year = "2015"
}

@article{Marsh:2015xka,
    author = "Marsh, David J. E.",
    title = "{Axion Cosmology}",
    eprint = "1510.07633",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "KCL-PH-TH-2015-50",
    doi = "10.1016/j.physrep.2016.06.005",
    journal = "Phys. Rept.",
    volume = "643",
    pages = "1--79",
    year = "2016"
}

@article{Graesser:2011wi,
    author = "Graesser, Michael L. and Shoemaker, Ian M. and Vecchi, Luca",
    title = "{Asymmetric WIMP dark matter}",
    eprint = "1103.2771",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "LA-UR-11-00565",
    doi = "10.1007/JHEP10(2011)110",
    journal = "JHEP",
    volume = "10",
    pages = "110",
    year = "2011"
}

@article{DOnofrio:2014rug,
    author = "D'Onofrio, Michela and Rummukainen, Kari and Tranberg, Anders",
    title = "{Sphaleron Rate in the Minimal Standard Model}",
    eprint = "1404.3565",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevLett.113.141602",
    journal = "Phys. Rev. Lett.",
    volume = "113",
    number = "14",
    pages = "141602",
    year = "2014"
}

@article{Shelton:2010ta,
    author = "Shelton, Jessie and Zurek, Kathryn M.",
    title = "{Darkogenesis: A baryon asymmetry from the dark matter sector}",
    eprint = "1008.1997",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MCTP-10-28",
    doi = "10.1103/PhysRevD.82.123512",
    journal = "Phys. Rev. D",
    volume = "82",
    pages = "123512",
    year = "2010"
}

@article{Wang:2019pet,
    author = "Wang, Xiao and Huang, Fa Peng and Zhang, Xinmin",
    title = "{Gravitational wave and collider signals in complex two-Higgs doublet model with dynamical CP-violation at finite temperature}",
    eprint = "1909.02978",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.101.015015",
    journal = "Phys. Rev. D",
    volume = "101",
    number = "1",
    pages = "015015",
    year = "2020"
}

@article{Carena:2004ha,
    author = "Carena, Marcela and Megevand, Ariel and Quiros, Mariano and Wagner, Carlos E.M.",
    title = "{Electroweak baryogenesis and new TeV fermions}",
    eprint = "hep-ph/0410352",
    archivePrefix = "arXiv",
    reportNumber = "ANL-HEP-PR-04-87, EFI-04-31, FERMILAB-PUB-04-264-T, UAB-FT-572",
    doi = "10.1016/j.nuclphysb.2005.03.025",
    journal = "Nucl. Phys. B",
    volume = "716",
    pages = "319--351",
    year = "2005"
}

@article{Prokopec:2003pj,
    author = "Prokopec, Tomislav and Schmidt, Michael G. and Weinstock, Steffen",
    title = "{Transport equations for chiral fermions to order h bar and electroweak baryogenesis. Part 1}",
    eprint = "hep-ph/0312110",
    archivePrefix = "arXiv",
    reportNumber = "BNL-72343-2004-JA, HD-THEP-03-62",
    doi = "10.1016/j.aop.2004.06.002",
    journal = "Annals Phys.",
    volume = "314",
    pages = "208--265",
    year = "2004"
}

@article{Prokopec:2004ic,
    author = "Prokopec, Tomislav and Schmidt, Michael G. and Weinstock, Steffen",
    title = "{Transport equations for chiral fermions to order h-bar and electroweak baryogenesis. Part II}",
    eprint = "hep-ph/0406140",
    archivePrefix = "arXiv",
    reportNumber = "BNL-72342-2004-JA, HD-THEP-04-22",
    doi = "10.1016/j.aop.2004.06.001",
    journal = "Annals Phys.",
    volume = "314",
    pages = "267--320",
    year = "2004"
}

@article{Elor:2020tkc,
    author = "Elor, Gilly and McGehee, Robert",
    title = "{Making the Universe at 20 MeV}",
    eprint = "2011.06115",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "11",
    year = "2020"
}

@article{Baldes:2017rcu,
    author = "Baldes, Iason",
    title = "{Gravitational waves from the asymmetric-dark-matter generating phase transition}",
    eprint = "1702.02117",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-17-021",
    doi = "10.1088/1475-7516/2017/05/028",
    journal = "JCAP",
    volume = "05",
    pages = "028",
    year = "2017"
}
@article{Petraki:2011mv,
    author = "Petraki, Kalliopi and Trodden, Mark and Volkas, Raymond R.",
    title = "{Visible and dark matter from a first-order phase transition in a baryon-symmetric universe}",
    eprint = "1111.4786",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2012/02/044",
    journal = "JCAP",
    volume = "02",
    pages = "044",
    year = "2012"
}

@article{Hall:2019rld,
    author = "Hall, Eleanor and Konstandin, Thomas and McGehee, Robert and Murayama, Hitoshi",
    title = "{Asymmetric Matters from a Dark First-Order Phase Transition}",
    eprint = "1911.12342",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IPMU19-0171, DESY-19-209",
    month = "11",
    year = "2019"
}

@article{Pilaftsis:1997jf,
    author = "Pilaftsis, Apostolos",
    title = "{CP violation and baryogenesis due to heavy Majorana neutrinos}",
    eprint = "hep-ph/9707235",
    archivePrefix = "arXiv",
    reportNumber = "MPI-PHT-97-30",
    doi = "10.1103/PhysRevD.56.5431",
    journal = "Phys. Rev. D",
    volume = "56",
    pages = "5431--5451",
    year = "1997"
}

@article{DAmbrosio:2003nfv,
    author = "D'Ambrosio, Giancarlo and Giudice, Gian F. and Raidal, Martti",
    title = "{Soft leptogenesis}",
    eprint = "hep-ph/0308031",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-2003-183, INFNNA-IV-03-30",
    doi = "10.1016/j.physletb.2003.09.037",
    journal = "Phys. Lett. B",
    volume = "575",
    pages = "75--84",
    year = "2003"
}

@article{Pilaftsis:2003gt,
    author = "Pilaftsis, Apostolos and Underwood, Thomas E. J.",
    title = "{Resonant leptogenesis}",
    eprint = "hep-ph/0309342",
    archivePrefix = "arXiv",
    reportNumber = "MC-TH-2003-09",
    doi = "10.1016/j.nuclphysb.2004.05.029",
    journal = "Nucl. Phys. B",
    volume = "692",
    pages = "303--345",
    year = "2004"
}
@article{Pilaftsis:1997jf,
    author = "Pilaftsis, Apostolos",
    title = "{CP violation and baryogenesis due to heavy Majorana neutrinos}",
    eprint = "hep-ph/9707235",
    archivePrefix = "arXiv",
    reportNumber = "MPI-PHT-97-30",
    doi = "10.1103/PhysRevD.56.5431",
    journal = "Phys. Rev. D",
    volume = "56",
    pages = "5431--5451",
    year = "1997"
}

@article{Abe:2019vii,
    author = "Abe, K. and others",
    collaboration = "T2K",
    title = "{Constraint on the matter\textendash{}antimatter symmetry-violating phase in neutrino oscillations}",
    eprint = "1910.03887",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    doi = "10.1038/s41586-020-2177-0",
    journal = "Nature",
    volume = "580",
    number = "7803",
    pages = "339--344",
    year = "2020",
    note = "[Erratum: Nature 583, E16 (2020)]"
}

@article{Acero:2019ksn,
    author = "Acero, M. A. and others",
    collaboration = "NOvA",
    title = "{First Measurement of Neutrino Oscillation Parameters using Neutrinos and Antineutrinos by NOvA}",
    eprint = "1906.04907",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "FERMILAB-PUB-19-272-ND",
    doi = "10.1103/PhysRevLett.123.151803",
    journal = "Phys. Rev. Lett.",
    volume = "123",
    number = "15",
    pages = "151803",
    year = "2019"
}

@article{Lazarides:1991wu,
    author = "Lazarides, George and Shafi, Q.",
    title = "{Origin of matter in the inflationary cosmology}",
    reportNumber = "BA-90-78",
    doi = "10.1016/0370-2693(91)91090-I",
    journal = "Phys. Lett. B",
    volume = "258",
    pages = "305--309",
    year = "1991"
}

@article{Asaka:1999yd,
    author = "Asaka, T. and Hamaguchi, Koichi and Kawasaki, M. and Yanagida, T.",
    title = "{Leptogenesis in inflaton decay}",
    eprint = "hep-ph/9906366",
    archivePrefix = "arXiv",
    reportNumber = "UT-853, RESCEU-15-99",
    doi = "10.1016/S0370-2693(99)01020-5",
    journal = "Phys. Lett. B",
    volume = "464",
    pages = "12--18",
    year = "1999"
}

@article{PhysRevD.67.043515,
  title = {Leptogenesis and rescattering in supersymmetric models},
  author = {Boubekeur, Lotfi and Davidson, Sacha and Peloso, Marco and Sorbo, Lorenzo},
  journal = {Phys. Rev. D},
  volume = {67},
  issue = {4},
  pages = {043515},
  numpages = {18},
  year = {2003},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.67.043515},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.67.043515}
}

@article{Giudice:1999fb,
    author = "Giudice, G. F. and Peloso, M. and Riotto, A. and Tkachev, I.",
    title = "{Production of massive fermions at preheating and leptogenesis}",
    eprint = "hep-ph/9905242",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-99-117",
    doi = "10.1088/1126-6708/1999/08/014",
    journal = "JHEP",
    volume = "08",
    pages = "014",
    year = "1999"
}

@article{Iminniyaz:2011yp,
    author = "Iminniyaz, Hoernisa and Drees, Manuel and Chen, Xuelei",
    title = "{Relic Abundance of Asymmetric Dark Matter}",
    eprint = "1104.5548",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2011/07/003",
    journal = "JCAP",
    volume = "07",
    pages = "003",
    year = "2011"
}


@article{Graesser:2011wi,
    author = "Graesser, Michael L. and Shoemaker, Ian M. and Vecchi, Luca",
    title = "{Asymmetric WIMP dark matter}",
    eprint = "1103.2771",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "LA-UR-11-00565",
    doi = "10.1007/JHEP10(2011)110",
    journal = "JHEP",
    volume = "10",
    pages = "110",
    year = "2011"
}

@article{Baker:2019ndr,
    author = "Baker, Michael J. and Kopp, Joachim and Long, Andrew J.",
    title = "{Filtered Dark Matter at a First Order Phase Transition}",
    eprint = "1912.02830",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevLett.125.151102",
    journal = "Phys. Rev. Lett.",
    volume = "125",
    number = "15",
    pages = "151102",
    year = "2020"
}
@article{Bodeker:2020ghk,
    author = "Bodeker, Dietrich and Buchmuller, Wilfried",
    title = "{Baryogenesis from the weak scale to the GUT scale}",
    eprint = "2009.07294",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-20-141",
    month = "9",
    year = "2020"
}

@article{Hooper:2020otu,
    author = "Hooper, Dan and Krnjaic, Gordan",
    title = "{GUT Baryogenesis With Primordial Black Holes}",
    eprint = "2010.01134",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-21-144-AE",
    doi = "10.1103/PhysRevD.103.043504",
    journal = "Phys. Rev. D",
    volume = "103",
    number = "4",
    pages = "043504",
    year = "2021"
}

@article{Nanopoulos:1979gx,
    author = "Nanopoulos, Dimitri V. and Weinberg, Steven",
    title = "{Mechanisms for Cosmological Baryon Production}",
    reportNumber = "HUTP-79/A023",
    doi = "10.1103/PhysRevD.20.2484",
    journal = "Phys. Rev. D",
    volume = "20",
    pages = "2484",
    year = "1979"
}

@article{Haba:2010bm,
    author = "Haba, N. and Matsumoto, S.",
    title = "{Baryogenesis from Dark Sector}",
    eprint = "1008.2487",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1143/PTP.125.1311",
    journal = "Prog. Theor. Phys.",
    volume = "125",
    pages = "1311--1316",
    year = "2011"
}

@article{Farrar:2005zd,
    author = "Farrar, Glennys R. and Zaharijas, Gabrijela",
    title = "{Dark matter and the baryon asymmetry}",
    eprint = "hep-ph/0510079",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevLett.96.041302",
    journal = "Phys. Rev. Lett.",
    volume = "96",
    pages = "041302",
    year = "2006"
}

@article{Baker:2019ndr,
    author = "Baker, Michael J. and Kopp, Joachim and Long, Andrew J.",
    title = "{Filtered Dark Matter at a First Order Phase Transition}",
    eprint = "1912.02830",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevLett.125.151102",
    journal = "Phys. Rev. Lett.",
    volume = "125",
    number = "15",
    pages = "151102",
    year = "2020"
}

@article{Creminelli:2001th,
    author = "Creminelli, Paolo and Nicolis, Alberto and Rattazzi, Riccardo",
    title = "{Holography and the electroweak phase transition}",
    eprint = "hep-th/0107141",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-2001-189",
    doi = "10.1088/1126-6708/2002/03/051",
    journal = "JHEP",
    volume = "03",
    pages = "051",
    year = "2002"
}

@article{Nardini:2007me,
    author = "Nardini, Germano and Quiros, Mariano and Wulzer, Andrea",
    title = "{A Confining Strong First-Order Electroweak Phase Transition}",
    eprint = "0706.3388",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UAB-FT-632",
    doi = "10.1088/1126-6708/2007/09/077",
    journal = "JHEP",
    volume = "09",
    pages = "077",
    year = "2007"
}




@article{EliasMiro:2011aa,
    author = "Elias-Miro, Joan and Espinosa, Jose R. and Giudice, Gian F. and Isidori, Gino and Riotto, Antonio and Strumia, Alessandro",
    title = "{Higgs mass implications on the stability of the electroweak vacuum}",
    eprint = "1112.3022",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1016/j.physletb.2012.02.013",
    journal = "Phys. Lett. B",
    volume = "709",
    pages = "222--228",
    year = "2012"
}

@article{Pascual-Dias:2020hxo,
    author = "Pascual-Dias, Bruna and Saha, Pratishruti and London, David",
    title = "{LHC Constraints on Scalar Diquarks}",
    eprint = "2006.13385",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UdeM-GPP-TH-20-279",
    doi = "10.1007/JHEP07(2020)144",
    journal = "JHEP",
    volume = "07",
    pages = "144",
    year = "2020"
}

@article{Davidson:2002qv,
    author = "Davidson, Sacha and Ibarra, Alejandro",
    title = "{A Lower bound on the right-handed neutrino mass from leptogenesis}",
    eprint = "hep-ph/0202239",
    archivePrefix = "arXiv",
    reportNumber = "OUTP-02-10P, IPPP-02-16, DCPT-02-32",
    doi = "10.1016/S0370-2693(02)01735-5",
    journal = "Phys. Lett. B",
    volume = "535",
    pages = "25--32",
    year = "2002"
}

@article{Phillips:2014fgb,
    author = "Phillips, II, D. G. and others",
    title = "{Neutron-Antineutron Oscillations: Theoretical Status and Experimental Prospects}",
    eprint = "1410.1100",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "FERMILAB-PUB-14-263-T",
    doi = "10.1016/j.physrep.2015.11.001",
    journal = "Phys. Rept.",
    volume = "612",
    pages = "1--45",
    year = "2016"
}

@article{Giudice:2011ak,
    author = "Giudice, Gian Francesco and Gripaios, Ben and Sundrum, Raman",
    title = "{Flavourful Production at Hadron Colliders}",
    eprint = "1105.3161",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-PH-TH-2011-110, UMD-PP-11-006",
    doi = "10.1007/JHEP08(2011)055",
    journal = "JHEP",
    volume = "08",
    pages = "055",
    year = "2011"
}
@article{Shuve:2017jgj,
    author = "Shuve, Brian and Tamarit, Carlos",
    title = "{Phase Transitions and Baryogenesis From Decays}",
    eprint = "1704.01979",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IPPP-17-17, SLAC-PUB-16942",
    doi = "10.1007/JHEP10(2017)122",
    journal = "JHEP",
    volume = "10",
    pages = "122",
    year = "2017"
}

@article{Chun:2023ezg,
    author = "Chun, Eung Jin and Dutka, Tomasz P. and Jung, Tae Hyun and Nagels, Xander and Vanvlasselaer, Miguel",
    title = "{Bubble-assisted leptogenesis}",
    eprint = "2305.10759",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CTPU-PTC-23-17",
    doi = "10.1007/JHEP09(2023)164",
    journal = "JHEP",
    volume = "09",
    pages = "164",
    year = "2023"
}


@article{Gouttenoire:2021kjv,
    author = "Gouttenoire, Yann and Jinno, Ryusuke and Sala, Filippo",
    title = "{Friction pressure on relativistic bubble walls}",
    eprint = "2112.07686",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-21-147, IFT-UAM/CSIC-21-146",
    doi = "10.1007/JHEP05(2022)004",
    journal = "JHEP",
    volume = "05",
    pages = "004",
    year = "2022"
}
@article{Azatov:2023xem,
    author = "Azatov, Aleksandr and Barni, Giulio and Petrossian-Byrne, Rudin and Vanvlasselaer, Miguel",
    title = "{Quantisation Across Bubble Walls and Friction}",
    eprint = "2310.06972",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SISSA 13/2023/FISI",
    month = "10",
    year = "2023"
}
@article{Ai:2023see,
    author = "Ai, Wen-Yuan and Laurent, Benoit and van de Vis, Jorinde",
    title = "{Model-independent bubble wall velocities in local thermal equilibrium}",
    eprint = "2303.10171",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "KCL-PH-TH/2023-19",
    doi = "10.1088/1475-7516/2023/07/002",
    journal = "JCAP",
    volume = "07",
    pages = "002",
    year = "2023"
}

@article{Ai:2024shx,
    author = "Ai, Wen-Yuan and Nagels, Xander and Vanvlasselaer, Miguel",
    title = "{Criterion for ultra-fast bubble walls: the impact of hydrodynamic obstruction}",
    eprint = "2401.05911",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KCL-PH-TH/2024-01",
    month = "1",
    year = "2024"
}
@article{FUKUGITA198645,
title = {Barygenesis without grand unification},
journal = {Physics Letters B},
volume = {174},
number = {1},
pages = {45-47},
year = {1986},
issn = {0370-2693},
doi = "https://doi.org/10.1016/0370-2693(86)91126-3",

author = "Fukugita , M and . Yanagida, T."},


@article{Ade:2015xua,
    author = "Ade, P. A. R. and others",
    collaboration = "Planck",
    title = "{Planck 2015 results. XIII. Cosmological parameters}",
    eprint = "1502.01589",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201525830",
    journal = "Astron. Astrophys.",
    volume = "594",
    pages = "A13",
    year = "2016"
}

@article{FUKUGITA198645,
title = {Barygenesis without grand unification},
journal = {Physics Letters B},
volume = {174},
number = {1},
pages = {45-47},
year = {1986},
issn = {0370-2693},
doi = "https://doi.org/10.1016/0370-2693(86)91126-3",

author = "Fukugita , M and . Yanagida, T."},


@article{Morrissey:2012db,
    author = "Morrissey, David E. and Ramsey-Musolf, Michael J.",
    title = "{Electroweak baryogenesis}",
    eprint = "1206.2942",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "NPAC-12-08",
    doi = "10.1088/1367-2630/14/12/125003",
    journal = "New J. Phys.",
    volume = "14",
    pages = "125003",
    year = "2012"
}

@article{Huet:1994jb,
    author = "Huet, Patrick and Sather, Eric",
    title = "{Electroweak baryogenesis and standard model CP violation}",
    eprint = "hep-ph/9404302",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-6479",
    doi = "10.1103/PhysRevD.51.379",
    journal = "Phys. Rev. D",
    volume = "51",
    pages = "379--394",
    year = "1995"
}

@article{Gavela:1994dt,
    author = "Gavela, M. B. and Hernandez, P. and Orloff, J. and Pene, O. and Quimbay, C.",
    title = "{Standard model CP violation and baryon asymmetry. Part 2: Finite temperature}",
    eprint = "hep-ph/9406289",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-7263-94, LPTHE-ORSAY-94-49, HUTP-94-A015, HD-THEP-94-20, FTUAM-94-14, NSF-ITP-94-65",
    doi = "10.1016/0550-3213(94)00410-2",
    journal = "Nucl. Phys. B",
    volume = "430",
    pages = "382--426",
    year = "1994"
}

@article{Gavela:1993ts,
    author = "Gavela, M. B. and Hernandez, P. and Orloff, J. and Pene, O.",
    title = "{Standard model CP violation and baryon asymmetry}",
    eprint = "hep-ph/9312215",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-7081-93, LPTHE-ORSAY-93-48, HUTP-93-A036, HD-THEP-93-45",
    doi = "10.1142/S0217732394000629",
    journal = "Mod. Phys. Lett. A",
    volume = "9",
    pages = "795--810",
    year = "1994"
}

@article{Kajantie:1995kf,
    author = "Kajantie, K. and Laine, M. and Rummukainen, K. and Shaposhnikov, Mikhail E.",
    title = "{The Electroweak phase transition: A Nonperturbative analysis}",
    eprint = "hep-lat/9510020",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-95-263, HD-THEP-95-44, HU-TFT-95-57, IUHET-318",
    doi = "10.1016/0550-3213(96)00052-1",
    journal = "Nucl. Phys. B",
    volume = "466",
    pages = "189--258",
    year = "1996"
}

@inproceedings{Cline:2006ts,
    author = "Cline, James M.",
    title = "{Baryogenesis}",
    booktitle = "{Les Houches Summer School - Session 86: Particle Physics and Cosmology: The Fabric of Spacetime}",
    eprint = "hep-ph/0609145",
    archivePrefix = "arXiv",
    month = "9",
    year = "2006"
}

@article{Bernreuther:2002uj,
    author = "Bernreuther, Werner",
    title = "{CP violation and baryogenesis}",
    eprint = "hep-ph/0205279",
    archivePrefix = "arXiv",
    reportNumber = "PITHA-02-08",
    journal = "Lect. Notes Phys.",
    volume = "591",
    pages = "237--293",
    year = "2002"
}
@article{Hamaguchi:2001gw,
    author = "Hamaguchi, Koichi and Murayama, Hitoshi and Yanagida, T.",
    title = "{Leptogenesis from N dominated early universe}",
    eprint = "hep-ph/0109030",
    archivePrefix = "arXiv",
    reportNumber = "UT-957, LBNL-48679, UCB-PTH-01-30",
    doi = "10.1103/PhysRevD.65.043512",
    journal = "Phys. Rev. D",
    volume = "65",
    pages = "043512",
    year = "2002"
}
@article{Fridell:2021gag,
    author = "Fridell, K\r{a}re and Harz, Julia and Hati, Chandan",
    title = "{Probing baryogenesis with neutron-antineutron oscillations}",
    eprint = "2105.06487",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "TUM-HEP-1337/21",
    month = "5",
    year = "2021"
}
@article{Omarov:2020kws,
    author = "Omarov, Zhanibek and Haciomeroglu, Selcuk and Lebedev, Valeri and Morse, William and Silenko, A. J. and Stephenson, E. J. and Semertzidis, Yannis K.",
    title = "{Comprehensive Symmetric-Hybrid ring design for pEDM experiment at below $10^{-29}e\cdot$cm}",
    eprint = "2007.10332",
    archivePrefix = "arXiv",
    primaryClass = "physics.acc-ph",
    month = "7",
    year = "2020"
}

@article{PhysRevD.45.3415,
  title = {Nucleation and bubble growth in a first-order cosmological electroweak phase transition},
  author = {Enqvist, K. and Ignatius, J. and Kajantie, K. and Rummukainen, K.},
  journal = {Phys. Rev. D},
  volume = {45},
  issue = {10},
  pages = {3415--3428},
  numpages = {0},
  year = {1992},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.45.3415},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.45.3415}
}

@article{Davidson:2008bu,
    author = "Davidson, Sacha and Nardi, Enrico and Nir, Yosef",
    title = "{Leptogenesis}",
    eprint = "0802.2962",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1016/j.physrep.2008.06.002",
    journal = "Phys. Rept.",
    volume = "466",
    pages = "105--177",
    year = "2008"
}



@article{Isidori:2010kg,
    author = "Isidori, Gino and Nir, Yosef and Perez, Gilad",
    title = "{Flavor Physics Constraints for Physics Beyond the Standard Model}",
    eprint = "1002.0900",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1146/annurev.nucl.012809.104534",
    journal = "Ann. Rev. Nucl. Part. Sci.",
    volume = "60",
    pages = "355",
    year = "2010"
}

@article{Chang:1990jv,
    author = "Chang, D. and Keung, Wai-Yee and Li, C. S. and Yuan, T. C.",
    title = "{{QCD} Corrections to {CP} Violation From Color Electric Dipole Moment of $b$ Quark}",
    reportNumber = "FERMILAB-PUB-90-038-T, UICPHY-TH-90-2, NUHEP-TH-90-7",
    doi = "10.1016/0370-2693(90)91875-C",
    journal = "Phys. Lett. B",
    volume = "241",
    pages = "589--592",
    year = "1990"
}

@article{Milstead:2015toa,
    author = "Milstead, David",
    title = "{A new high sensitivity search for neutron-antineutron oscillations at the ESS}",
    eprint = "1510.01569",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    doi = "10.22323/1.234.0603",
    journal = "PoS",
    volume = "EPS-HEP2015",
    pages = "603",
    year = "2015"
}

@phdthesis{Hewes:2017xtr,
    author = "Hewes, Jeremy E. T.",
    title = "{Searches for Bound Neutron-Antineutron Oscillation in Liquid Argon Time Projection Chambers}",
    reportNumber = "FERMILAB-THESIS-2017-27",
    doi = "10.2172/1426674",
    school = "Manchester U.",
    year = "2017"
}

@article{Rao:1982gt,
    author = "Rao, Sumathi and Shrock, Robert",
    title = "{$n \leftrightarrow \bar{n}$ Transition Operators and Their Matrix Elements in the {MIT} Bag Model}",
    reportNumber = "ITP-SB-82-28",
    doi = "10.1016/0370-2693(82)90333-1",
    journal = "Phys. Lett. B",
    volume = "116",
    pages = "238--242",
    year = "1982"
}
@article{Syritsyn:2016ijx,
    author = "Syritsyn, Sergey and Buchoff, Michael I and Schroeder, Chris and Wasem, Joseph",
    title = "{Neutron-antineutron oscillation matrix elements with domain wall fermions at the physical point}",
    doi = "10.22323/1.251.0132",
    journal = "PoS",
    volume = "LATTICE2015",
    pages = "132",
    year = "2016"
}

@article{Ma:2006km,
    author = "Ma, Ernest",
    title = "{Verifiable radiative seesaw mechanism of neutrino mass and dark matter}",
    eprint = "hep-ph/0601225",
    archivePrefix = "arXiv",
    reportNumber = "UCRHEP-T403",
    doi = "10.1103/PhysRevD.73.077301",
    journal = "Phys. Rev. D",
    volume = "73",
    pages = "077301",
    year = "2006"
}

@article{Glashow:1979nm,
    author = "Glashow, S. L.",
    title = "{The Future of Elementary Particle Physics}",
    reportNumber = "HUTP-79-A059",
    doi = "10.1007/978-1-4684-7197-7_15",
    journal = "NATO Sci. Ser. B",
    volume = "61",
    pages = "687",
    year = "1980"
}
@article{Barbier:2004ez,
    author = "Barbier, R. and others",
    title = "{R-parity violating supersymmetry}",
    eprint = "hep-ph/0406039",
    archivePrefix = "arXiv",
    doi = "10.1016/j.physrep.2005.08.006",
    journal = "Phys. Rept.",
    volume = "420",
    pages = "1--202",
    year = "2005"
}
@article{Babu:2006xc,
    author = "Babu, K. S. and Mohapatra, R. N. and Nasri, S.",
    title = "{Post-Sphaleron Baryogenesis}",
    eprint = "hep-ph/0606144",
    archivePrefix = "arXiv",
    reportNumber = "UMD-PP-06-004, OSU-HEP-06-02",
    doi = "10.1103/PhysRevLett.97.131301",
    journal = "Phys. Rev. Lett.",
    volume = "97",
    pages = "131301",
    year = "2006"
}
@article{McKeen:2015cuz,
    author = "McKeen, David and Nelson, Ann E.",
    title = "{CP Violating Baryon Oscillations}",
    eprint = "1512.05359",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.94.076002",
    journal = "Phys. Rev. D",
    volume = "94",
    number = "7",
    pages = "076002",
    year = "2016"
}

@article{Aitken:2017wie,
    author = "Aitken, Kyle and McKeen, David and Neder, Thomas and Nelson, Ann E.",
    title = "{Baryogenesis from Oscillations of Charmed or Beautiful Baryons}",
    eprint = "1708.01259",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PITT-PACC-1709",
    doi = "10.1103/PhysRevD.96.075009",
    journal = "Phys. Rev. D",
    volume = "96",
    number = "7",
    pages = "075009",
    year = "2017"
}

@article{Elor:2018twp,
    author = "Elor, Gilly and Escudero, Miguel and Nelson, Ann",
    title = "{Baryogenesis and Dark Matter from $B$ Mesons}",
    eprint = "1810.00880",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KCL-18-53, IFIC-18-35",
    doi = "10.1103/PhysRevD.99.035031",
    journal = "Phys. Rev. D",
    volume = "99",
    number = "3",
    pages = "035031",
    year = "2019"
}

@article{Grojean:2018fus,
    author = "Grojean, Christophe and Shakya, Bibhushan and Wells, James D. and Zhang, Zhengkang",
    title = "{Implications of an Improved Neutron-Antineutron Oscillation Search for Baryogenesis: A Minimal Effective Theory Analysis}",
    eprint = "1806.00011",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-18-062, LCTP-18-14",
    doi = "10.1103/PhysRevLett.121.171801",
    journal = "Phys. Rev. Lett.",
    volume = "121",
    number = "17",
    pages = "171801",
    year = "2018"
}

@article{Hamada:2018epb,
    author = "Hamada, Yuta and Kitano, Ryuichiro and Yin, Wen",
    title = "{Leptogenesis via Neutrino Oscillation Magic}",
    eprint = "1807.06582",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KEK-TH-2064",
    doi = "10.1007/JHEP10(2018)178",
    journal = "JHEP",
    volume = "10",
    pages = "178",
    year = "2018"
}

@article{Pierce:2019ozl,
    author = "Pierce, Aaron and Shakya, Bibhushan",
    title = "{Gaugino Portal Baryogenesis}",
    eprint = "1901.05493",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "LCTP-19-01",
    doi = "10.1007/JHEP06(2019)096",
    journal = "JHEP",
    volume = "06",
    pages = "096",
    year = "2019"
}

@article{Asaka:2019ocw,
    author = "Asaka, Takehiko and Ishida, Hiroyuki and Yin, Wen",
    title = "{Direct baryogenesis in the broken phase}",
    eprint = "1912.08797",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KEK-TH-2179",
    doi = "10.1007/JHEP07(2020)174",
    journal = "JHEP",
    volume = "07",
    pages = "174",
    year = "2020"
}
@article{Cao:2021yau,
    author = "Cao, Qing-Hong and Hashino, Katsuya and Li, Xu-Xiang and Ren, Zhe and Yu, Jiang-Hao",
    title = "{Electroweak phase transition triggered by fermion sector}",
    eprint = "2103.05688",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2021"
}

@article{Baldes:2016rqn,
    author = "Baldes, Iason and Konstandin, Thomas and Servant, Geraldine",
    title = "{A first-order electroweak phase transition from varying Yukawas}",
    eprint = "1604.04526",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-16-068",
    doi = "10.1016/j.physletb.2018.10.015",
    journal = "Phys. Lett. B",
    volume = "786",
    pages = "373--377",
    year = "2018"
}
@article{Craig:2020jfv,
    author = "Craig, Nathaniel and Levi, Noam and Mariotti, Alberto and Redigolo, Diego",
    title = "{Ripples in Spacetime from Broken Supersymmetry}",
    eprint = "2011.13949",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP02(2021)184",
    journal = "JHEP",
    volume = "21",
    pages = "184",
    year = "2020"
}

@article{Brivio:2017dfq,
    author = "Brivio, Ilaria and Trott, Michael",
    title = "{Radiatively Generating the Higgs Potential and Electroweak Scale via the Seesaw Mechanism}",
    eprint = "1703.10924",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevLett.119.141801",
    journal = "Phys. Rev. Lett.",
    volume = "119",
    number = "14",
    pages = "141801",
    year = "2017"
}
@article{Engel:2013lsa,
    author = "Engel, Jonathan and Ramsey-Musolf, Michael J. and van Kolck, U.",
    title = "{Electric Dipole Moments of Nucleons, Nuclei, and Atoms: The Standard Model and Beyond}",
    eprint = "1303.2371",
    archivePrefix = "arXiv",
    primaryClass = "nucl-th",
    doi = "10.1016/j.ppnp.2013.03.003",
    journal = "Prog. Part. Nucl. Phys.",
    volume = "71",
    pages = "21--74",
    year = "2013"
}

@article{Baldes:2021vyz,
    author = "Baldes, Iason and Blasi, Simone and Mariotti, Alberto and Sevrin, Alexander and Turbang, Kevin",
    title = "{Baryogenesis via relativistic bubble expansion}",
    eprint = "2106.15602",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "ULB-TH/21-09",
    month = "6",
    year = "2021"
}

@article{Jinno:2019bxw,
    author = "Jinno, Ryusuke and Konstandin, Thomas and Takimoto, Masahiro",
    title = "{Relativistic bubble collisions-a closer look}",
    eprint = "1906.02588",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-19-102, DESY 19-102",
    doi = "10.1088/1475-7516/2019/09/035",
    journal = "JCAP",
    volume = "09",
    pages = "035",
    year = "2019"
}

@article{Dorsch:2021ubz,
    author = "Dorsch, Glauber C. and Huber, Stephan J. and Konstandin, Thomas",
    title = "{On the wall velocity dependence of electroweak baryogenesis}",
    eprint = "2106.06547",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-21-089",
    month = "6",
    year = "2021"
}

@article{Badurina:2019hst,
    author = "Badurina, L. and others",
    title = "{AION: An Atom Interferometer Observatory and Network}",
    eprint = "1911.11755",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "AION-2019-001, CERN-TH-2019-199",
    doi = "10.1088/1475-7516/2020/05/011",
    journal = "JCAP",
    volume = "05",
    pages = "011",
    year = "2020"
}
@article{Bertoldi:2019tck,
    author = "El-Neaj, Yousef Abou and others",
    collaboration = "AEDGE",
    title = "{AEDGE: Atomic Experiment for Dark Matter and Gravity Exploration in Space}",
    eprint = "1908.00802",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    reportNumber = "KCL-PH-TH/2019-65, CERN-TH-2019-126",
    doi = "10.1140/epjqt/s40507-020-0080-0",
    journal = "EPJ Quant. Technol.",
    volume = "7",
    pages = "6",
    year = "2020"
}
@article{Maggiore:2019uih,
    author = "Maggiore, Michele and others",
    title = "{Science Case for the Einstein Telescope}",
    eprint = "1912.02622",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2020/03/050",
    journal = "JCAP",
    volume = "03",
    pages = "050",
    year = "2020"
}


@article{Hild:2010id,
    author = "Hild, S. and others",
    title = "{Sensitivity Studies for Third-Generation Gravitational Wave Observatories}",
    eprint = "1012.0908",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/0264-9381/28/9/094013",
    journal = "Class. Quant. Grav.",
    volume = "28",
    pages = "094013",
    year = "2011"
}
@article{Crowder:2005nr,
    author = "Crowder, Jeff and Cornish, Neil J.",
    title = "{Beyond LISA: Exploring future gravitational wave missions}",
    eprint = "gr-qc/0506015",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.72.083005",
    journal = "Phys. Rev. D",
    volume = "72",
    pages = "083005",
    year = "2005"
}
@article{Corbin:2005ny,
    author = "Corbin, Vincent and Cornish, Neil J.",
    title = "{Detecting the cosmic gravitational wave background with the big bang observer}",
    eprint = "gr-qc/0512039",
    archivePrefix = "arXiv",
    doi = "10.1088/0264-9381/23/7/014",
    journal = "Class. Quant. Grav.",
    volume = "23",
    pages = "2435--2446",
    year = "2006"
}

@article{Isoyama:2018rjb,
    author = "Isoyama, Soichiro and Nakano, Hiroyuki and Nakamura, Takashi",
    title = "{Multiband Gravitational-Wave Astronomy: Observing binary inspirals with a decihertz detector, B-DECIGO}",
    eprint = "1802.06977",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1093/ptep/pty078",
    journal = "PTEP",
    volume = "2018",
    number = "7",
    pages = "073E01",
    year = "2018"
}

@article{Yagi:2011wg,
    author = "Yagi, Kent and Seto, Naoki",
    title = "{Detector configuration of DECIGO/BBO and identification of cosmological neutron-star binaries}",
    eprint = "1101.3940",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.83.044011",
    journal = "Phys. Rev. D",
    volume = "83",
    pages = "044011",
    year = "2011",
    note = "[Erratum: Phys.Rev.D 95, 109901 (2017)]"
}

@article{Seto:2001qf,
    author = "Seto, Naoki and Kawamura, Seiji and Nakamura, Takashi",
    title = "{Possibility of direct measurement of the acceleration of the universe using 0.1-Hz band laser interferometer gravitational wave antenna in space}",
    eprint = "astro-ph/0108011",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevLett.87.221103",
    journal = "Phys. Rev. Lett.",
    volume = "87",
    pages = "221103",
    year = "2001"
}

@misc{amaroseoane2017laser,
      title={Laser Interferometer Space Antenna}, 
      author={Pau Amaro-Seoane and Heather Audley and Stanislav Babak and John Baker and Enrico Barausse and Peter Bender and Emanuele Berti and Pierre Binetruy and Michael Born and Daniele Bortoluzzi and Jordan Camp and Chiara Caprini and Vitor Cardoso and Monica Colpi and John Conklin and Neil Cornish and Curt Cutler and Karsten Danzmann and Rita Dolesi and Luigi Ferraioli and Valerio Ferroni and Ewan Fitzsimons and Jonathan Gair and Lluis Gesa Bote and Domenico Giardini and Ferran Gibert and Catia Grimani and Hubert Halloin and Gerhard Heinzel and Thomas Hertog and Martin Hewitson and Kelly Holley-Bockelmann and Daniel Hollington and Mauro Hueller and Henri Inchauspe and Philippe Jetzer and Nikos Karnesis and Christian Killow and Antoine Klein and Bill Klipstein and Natalia Korsakova and Shane L Larson and Jeffrey Livas and Ivan Lloro and Nary Man and Davor Mance and Joseph Martino and Ignacio Mateos and Kirk McKenzie and Sean T McWilliams and Cole Miller and Guido Mueller and Germano Nardini and Gijs Nelemans and Miquel Nofrarias and Antoine Petiteau and Paolo Pivato and Eric Plagnol and Ed Porter and Jens Reiche and David Robertson and Norna Robertson and Elena Rossi and Giuliana Russano and Bernard Schutz and Alberto Sesana and David Shoemaker and Jacob Slutsky and Carlos F. Sopuerta and Tim Sumner and Nicola Tamanini and Ira Thorpe and Michael Troebs and Michele Vallisneri and Alberto Vecchio and Daniele Vetrugno and Stefano Vitale and Marta Volonteri and Gudrun Wanner and Harry Ward and Peter Wass and William Weber and John Ziemer and Peter Zweifel},
      year={2017},
      eprint={1702.00786},
      archivePrefix={arXiv},
      primaryClass={astro-ph.IM}
}

@article{Brdar:2018num,
    author = "Brdar, Vedran and Helmboldt, Alexander J. and Kubo, Jisuke",
    title = "{Gravitational Waves from First-Order Phase Transitions: LIGO as a Window to Unexplored Seesaw Scales}",
    eprint = "1810.12306",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2019/02/021",
    journal = "JCAP",
    volume = "02",
    pages = "021",
    year = "2019"
}

@article{vonHarling:2019gme,
    author = "Von Harling, Benedict and Pomarol, Alex and Pujol\`as, Oriol and Rompineve, Fabrizio",
    title = "{Peccei-Quinn Phase Transition at LIGO}",
    eprint = "1912.07587",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP04(2020)195",
    journal = "JHEP",
    volume = "04",
    pages = "195",
    year = "2020"
}



@article{Weir:2017wfa,
    author = "Weir, David J.",
    title = "{Gravitational waves from a first order electroweak phase transition: a brief review}",
    eprint = "1705.01783",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "HIP-2017-06-TH",
    doi = "10.1098/rsta.2017.0126",
    journal = "Phil. Trans. Roy. Soc. Lond. A",
    volume = "376",
    number = "2114",
    pages = "20170126",
    year = "2018"
}
@article{Davoudiasl:2021vku,
    author = "Davoudiasl, Hooman",
    title = "{First Order Electroweak Phase Transition from Weakly Coupled sub-GeV Physics and Possible Connection to Fermion Flavor}",
    eprint = "2101.05319",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.103.083534",
    journal = "Phys. Rev. D",
    volume = "103",
    number = "8",
    pages = "083534",
    year = "2021"
}

@article{Andreev:2018ayy,
    author = "Andreev, V. and others",
    collaboration = "ACME",
    title = "{Improved limit on the electric dipole moment of the electron}",
    doi = "10.1038/s41586-018-0599-8",
    journal = "Nature",
    volume = "562",
    number = "7727",
    pages = "355--360",
    year = "2018"
}

@article{Harvey:1990qw,
    author = "Harvey, Jeffrey A. and Turner, Michael S.",
    title = "{Cosmological baryon and lepton number in the presence of electroweak fermion number violation}",
    reportNumber = "FERMILAB-PUB-90-049-A, EFI-90-33",
    doi = "10.1103/PhysRevD.42.3344",
    journal = "Phys. Rev. D",
    volume = "42",
    pages = "3344--3349",
    year = "1990"
}


@article{Charnock:2016nzm,
    author = "Charnock, Tom and Avgoustidis, Anastasios and Copeland, Edmund J. and Moss, Adam",
    title = "{CMB constraints on cosmic strings and superstrings}",
    eprint = "1603.01275",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.93.123503",
    journal = "Phys. Rev. D",
    volume = "93",
    number = "12",
    pages = "123503",
    year = "2016"
}
@article{Su:2020pjw,
    author = "Su, Wei and Williams, Anthony G. and Zhang, Mengchao",
    title = "{Strong first order electroweak phase transition in 2HDM confronting future Z \& Higgs factories}",
    eprint = "2011.04540",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "ADP-20-31/T1141",
    doi = "10.1007/JHEP04(2021)219",
    journal = "JHEP",
    volume = "04",
    pages = "219",
    year = "2021"
}






@article{Eichhorn:2020upj,
    author = "Eichhorn, Astrid and Lumma, Johannes and Pawlowski, Jan M. and Reichert, Manuel and Yamada, Masatoshi",
    title = "{Universal gravitational-wave signatures from heavy new physics in the electroweak sector}",
    eprint = "2010.00017",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2021/05/006",
    journal = "JCAP",
    volume = "05",
    pages = "006",
    year = "2021"
}
@article{Camargo-Molina:2021zcp,
    author = {Camargo-Molina, Jos\'e Eliel and Enberg, Rikard and L\"ofgren, Johan},
    title = "{A new perspective on the electroweak phase transition in the Standard Model Effective Field Theory}",
    eprint = "2103.14022",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2021"
}
@article{Grojean:2004xa,
    author = "Grojean, Christophe and Servant, Geraldine and Wells, James D.",
    title = "{First-order electroweak phase transition in the standard model with a low cutoff}",
    eprint = "hep-ph/0407019",
    archivePrefix = "arXiv",
    reportNumber = "SACLAY-T04-084, MCTP-04-37, ANL-HEP-PR-04-63, EFI-04-23",
    doi = "10.1103/PhysRevD.71.036001",
    journal = "Phys. Rev. D",
    volume = "71",
    pages = "036001",
    year = "2005"
}




@article{Dimopoulos:1987rk,
    author = "Dimopoulos, Savas and Hall, Lawrence J.",
    title = "{Baryogenesis at the {MeV} Era}",
    reportNumber = "LBL-23516",
    doi = "10.1016/0370-2693(87)90593-4",
    journal = "Phys. Lett. B",
    volume = "196",
    pages = "135--141",
    year = "1987"
}
@article{Mohapatra:1979ia,
    author = "Mohapatra, Rabindra N. and Senjanovic, Goran",
    title = "{Neutrino Mass and Spontaneous Parity Nonconservation}",
    reportNumber = "MDDP-TR-80-060, MDDP-PP-80-105, CCNY-HEP-79-10",
    doi = "10.1103/PhysRevLett.44.912",
    journal = "Phys. Rev. Lett.",
    volume = "44",
    pages = "912",
    year = "1980"
}

@article{GellMann:1980vs,
    author = "Gell-Mann, Murray and Ramond, Pierre and Slansky, Richard",
    title = "{Complex Spinors and Unified Theories}",
    eprint = "1306.4669",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "PRINT-80-0576",
    journal = "Conf. Proc. C",
    volume = "790927",
    pages = "315--321",
    year = "1979"
}

@article{Yanagida:1979as,
    author = "Yanagida, Tsutomu",
    editor = "Sawada, Osamu and Sugamoto, Akio",
    title = "{Horizontal gauge symmetry and masses of neutrinos}",
    reportNumber = "KEK-79-18-95",
    journal = "Conf. Proc. C",
    volume = "7902131",
    pages = "95--99",
    year = "1979"
}

@article{Minkowski:1977sc,
    author = "Minkowski, Peter",
    title = "{$\mu \to e\gamma$ at a Rate of One Out of $10^{9}$ Muon Decays?}",
    reportNumber = "Print-77-0182 (BERN)",
    doi = "10.1016/0370-2693(77)90435-X",
    journal = "Phys. Lett. B",
    volume = "67",
    pages = "421--428",
    year = "1977"
}

@article{Fukugita:1986hr,
    author = "Fukugita, M. and Yanagida, T.",
    title = "{Baryogenesis Without Grand Unification}",
    reportNumber = "RIFP-641",
    doi = "10.1016/0370-2693(86)91126-3",
    journal = "Phys. Lett. B",
    volume = "174",
    pages = "45--47",
    year = "1986"
}

@article{Buchoff:2012bm,
    author = "Buchoff, Michael I. and Schroeder, Chris and Wasem, Joseph",
    title = "{Neutron-antineutron oscillations on the lattice}",
    eprint = "1207.3832",
    archivePrefix = "arXiv",
    primaryClass = "hep-lat",
    reportNumber = "LLNL-PROC-563736",
    doi = "10.22323/1.164.0128",
    journal = "PoS",
    volume = "LATTICE2012",
    pages = "128",
    year = "2012"
}

@article{Abe:2011ky,
    author = "Abe, K. and others",
    collaboration = "Super-Kamiokande",
    title = "{The Search for $n-\bar{n}$ oscillation in Super-Kamiokande I}",
    eprint = "1109.4227",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    doi = "10.1103/PhysRevD.91.072006",
    journal = "Phys. Rev. D",
    volume = "91",
    pages = "072006",
    year = "2015"
}

@article{BaldoCeolin:1994jz,
    author = "Baldo-Ceolin, M. and others",
    title = "{A New experimental limit on neutron - anti-neutron oscillations}",
    reportNumber = "DFPD-94-EP-13",
    doi = "10.1007/BF01580321",
    journal = "Z. Phys. C",
    volume = "63",
    pages = "409--416",
    year = "1994"
}

@inproceedings{Frost:2016qzt,
    author = "Frost, M. J.",
    collaboration = "NNbar",
    title = "{The NNbar Experiment at the European Spallation Source}",
    booktitle = "{7th Meeting on CPT and Lorentz Symmetry}",
    eprint = "1607.07271",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1142/9789813148505_0070",
    month = "7",
    year = "2016"
}

@article{Sirunyan:2019ctn,
    author = "Sirunyan, Albert M and others",
    collaboration = "CMS",
    title = "{Search for supersymmetry in proton-proton collisions at 13 TeV in final states with jets and missing transverse momentum}",
    eprint = "1908.04722",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-SUS-19-006, CERN-EP-2019-152",
    doi = "10.1007/JHEP10(2019)244",
    journal = "JHEP",
    volume = "10",
    pages = "244",
    year = "2019"
}

@article{Aad:2020aze,
    author = "Aad, Georges and others",
    collaboration = "ATLAS",
    title = "{Search for squarks and gluinos in final states with jets and missing transverse momentum using 139 fb$^{-1}$ of $\sqrt{s}$ =13 TeV $pp$ collision data with the ATLAS detector}",
    eprint = "2010.14293",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2020-166",
    doi = "10.1007/JHEP02(2021)143",
    journal = "JHEP",
    volume = "02",
    pages = "143",
    year = "2021"
}
